Signing in Four Public Software Package Registries: Quantity, Quality, and Influencing Factors

Many software applications incorporate open-source third-party packages distributed by public package registries. Guaranteeing authorship along this supply chain is a challenge. Package maintainers can guarantee package authorship through software signing. However, it is unclear how common this practice is, and whether the resulting signatures are created properly. Prior work has provided raw data on registry signing practices, but only measured single platforms, did not consider quality, did not consider time, and did not assess factors that may influence signing. We do not have up-to-date measurements of signing practices nor do we know the quality of existing signatures. Furthermore, we lack a comprehensive understanding of factors that influence signing adoption. This study addresses this gap. We provide measurements across three kinds of package registries: traditional software (Maven, PyPI), container images (DockerHub), and machine learning models (Hugging Face). For each registry, we describe the nature of the signed artifacts as well as the current quantity and quality of signatures. Then, we examine longitudinal trends in signing practices. Finally, we use a quasi-experiment to estimate the effect that various factors had on software signing practices. To summarize our findings: (1) mandating signature adoption improves the quantity of signatures; (2) providing dedicated tooling improves the quality of signing; (3) getting started is the hard part -- once a maintainer begins to sign, they tend to continue doing so; and (4) although many supply chain attacks are mitigable via signing, signing adoption is primarily affected by registry policy rather than by public knowledge of attacks, new engineering standards, etc. These findings highlight the importance of software package registry managers and signing infrastructure.

==> data/crypto.tex <==
\makeatletter\newcommand\crypto[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@out{\{"maven": \{"ecdsa": \{"count": 952, "human": "952", "percent": "0.01\%"\}, "rsasignonly": \{"count": 2449, "human": "2.45K", "percent": "0.03\%"\}, "dsa": \{"count": 134375, "human": "134K", "percent": "1.79\%"\}, "eddsa": \{"count": 161363, "human": "161K", "percent": "2.15\%"\}, "rsa": \{"count": 7198053, "human": "7.2M", "percent": "96.01\%", "key\_sizes": \{"1536": \{"count": 20, "human": "20", "percent": "0.000\%"\}, "2560": \{"count": 142, "human": "142", "percent": "0.002\%"\}, "8192": \{"count": 374, "human": "374", "percent": "0.005\%"\}, "4608": \{"count": 402, "human": "402", "percent": "0.006\%"\}, "1024": \{"count": 19529, "human": "19.5K", "percent": "0.271\%"\}, "3072": \{"count": 999944, "human": "1M", "percent": "13.892\%"\}, "4096": \{"count": 2746911, "human": "2.75M", "percent": "38.162\%"\}, "2048": \{"count": 3430731, "human": "3.43M", "percent": "47.662\%"\}\}\}\}, "pypi": \{"ecdsa": \{"count": 310, "human": "310", "percent": "0.26\%"\}, "eddsa": \{"count": 3260, "human": "3.26K", "percent": "2.71\%"\}, "dsa": \{"count": 13519, "human": "13.5K", "percent": "11.22\%"\}, "rsa": \{"count": 103423, "human": "103K", "percent": "85.82\%", "key\_sizes": \{"1536": \{"count": 1, "human": "1", "percent": "0.001\%"\}, "8192": \{"count": 147, "human": "147", "percent": "0.142\%"\}, "1024": \{"count": 148, "human": "148", "percent": "0.143\%"\}, "3072": \{"count": 2248, "human": "2.25K", "percent": "2.174\%"\}, "2048": \{"count": 49874, "human": "49.9K", "percent": "48.223\%"\}, "4096": \{"count": 51005, "human": "51K", "percent": "49.317\%"\}, "2560": \{"count": 0, "human": "0", "percent": "0.000\%"\}, "4608": \{"count": 0, "human": "0", "percent": "0.000\%"\}\}\}, "rsasignonly": \{"count": 0, "human": "0", "percent": "0.00\%"\}\}\}}\else\ifnum\pdfstrcmp{#1}{maven}=0\let\crypto@out\crypto@I\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\crypto@out\crypto@II\else\def\crypto@out{??}\fi\fi\fi\crypto@out}\newcommand\crypto@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@I@out{\{"ecdsa": \{"count": 952, "human": "952", "percent": "0.01\%"\}, "rsasignonly": \{"count": 2449, "human": "2.45K", "percent": "0.03\%"\}, "dsa": \{"count": 134375, "human": "134K", "percent": "1.79\%"\}, "eddsa": \{"count": 161363, "human": "161K", "percent": "2.15\%"\}, "rsa": \{"count": 7198053, "human": "7.2M", "percent": "96.01\%", "key\_sizes": \{"1536": \{"count": 20, "human": "20", "percent": "0.000\%"\}, "2560": \{"count": 142, "human": "142", "percent": "0.002\%"\}, "8192": \{"count": 374, "human": "374", "percent": "0.005\%"\}, "4608": \{"count": 402, "human": "402", "percent": "0.006\%"\}, "1024": \{"count": 19529, "human": "19.5K", "percent": "0.271\%"\}, "3072": \{"count": 999944, "human": "1M", "percent": "13.892\%"\}, "4096": \{"count": 2746911, "human": "2.75M", "percent": "38.162\%"\}, "2048": \{"count": 3430731, "human": "3.43M", "percent": "47.662\%"\}\}\}\}}\else\ifnum\pdfstrcmp{#1}{ecdsa}=0\let\crypto@I@out\crypto@III\else\ifnum\pdfstrcmp{#1}{rsasignonly}=0\let\crypto@I@out\crypto@IV\else\ifnum\pdfstrcmp{#1}{dsa}=0\let\crypto@I@out\crypto@V\else\ifnum\pdfstrcmp{#1}{eddsa}=0\let\crypto@I@out\crypto@VI\else\ifnum\pdfstrcmp{#1}{rsa}=0\let\crypto@I@out\crypto@VII\else\def\crypto@I@out{??}\fi\fi\fi\fi\fi\fi\crypto@I@out}\newcommand\crypto@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@II@out{\{"ecdsa": \{"count": 310, "human": "310", "percent": "0.26\%"\}, "eddsa": \{"count": 3260, "human": "3.26K", "percent": "2.71\%"\}, "dsa": \{"count": 13519, "human": "13.5K", "percent": "11.22\%"\}, "rsa": \{"count": 103423, "human": "103K", "percent": "85.82\%", "key\_sizes": \{"1536": \{"count": 1, "human": "1", "percent": "0.001\%"\}, "8192": \{"count": 147, "human": "147", "percent": "0.142\%"\}, "1024": \{"count": 148, "human": "148", "percent": "0.143\%"\}, "3072": \{"count": 2248, "human": "2.25K", "percent": "2.174\%"\}, "2048": \{"count": 49874, "human": "49.9K", "percent": "48.223\%"\}, "4096": \{"count": 51005, "human": "51K", "percent": "49.317\%"\}, "2560": \{"count": 0, "human": "0", "percent": "0.000\%"\}, "4608": \{"count": 0, "human": "0", "percent": "0.000\%"\}\}\}, "rsasignonly": \{"count": 0, "human": "0", "percent": "0.00\%"\}\}}\else\ifnum\pdfstrcmp{#1}{ecdsa}=0\let\crypto@II@out\crypto@VIII\else\ifnum\pdfstrcmp{#1}{eddsa}=0\let\crypto@II@out\crypto@IX\else\ifnum\pdfstrcmp{#1}{dsa}=0\let\crypto@II@out\crypto@X\else\ifnum\pdfstrcmp{#1}{rsa}=0\let\crypto@II@out\crypto@XI\else\ifnum\pdfstrcmp{#1}{rsasignonly}=0\let\crypto@II@out\crypto@XII\else\def\crypto@II@out{??}\fi\fi\fi\fi\fi\fi\crypto@II@out}\newcommand\crypto@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@III@out{\{"count": 952, "human": "952", "percent": "0.01\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@III@out{952}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@III@out{952}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@III@out{0.01\%}\else\def\crypto@III@out{??}\fi\fi\fi\fi\crypto@III@out}\newcommand\crypto@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@IV@out{\{"count": 2449, "human": "2.45K", "percent": "0.03\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@IV@out{2449}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@IV@out{2.45K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@IV@out{0.03\%}\else\def\crypto@IV@out{??}\fi\fi\fi\fi\crypto@IV@out}\newcommand\crypto@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@V@out{\{"count": 134375, "human": "134K", "percent": "1.79\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@V@out{134375}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@V@out{134K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@V@out{1.79\%}\else\def\crypto@V@out{??}\fi\fi\fi\fi\crypto@V@out}\newcommand\crypto@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@VI@out{\{"count": 161363, "human": "161K", "percent": "2.15\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@VI@out{161363}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@VI@out{161K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@VI@out{2.15\%}\else\def\crypto@VI@out{??}\fi\fi\fi\fi\crypto@VI@out}\newcommand\crypto@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@VII@out{\{"count": 7198053, "human": "7.2M", "percent": "96.01\%", "key\_sizes": \{"1536": \{"count": 20, "human": "20", "percent": "0.000\%"\}, "2560": \{"count": 142, "human": "142", "percent": "0.002\%"\}, "8192": \{"count": 374, "human": "374", "percent": "0.005\%"\}, "4608": \{"count": 402, "human": "402", "percent": "0.006\%"\}, "1024": \{"count": 19529, "human": "19.5K", "percent": "0.271\%"\}, "3072": \{"count": 999944, "human": "1M", "percent": "13.892\%"\}, "4096": \{"count": 2746911, "human": "2.75M", "percent": "38.162\%"\}, "2048": \{"count": 3430731, "human": "3.43M", "percent": "47.662\%"\}\}\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@VII@out{7198053}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@VII@out{7.2M}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@VII@out{96.01\%}\else\ifnum\pdfstrcmp{#1}{key_sizes}=0\let\crypto@VII@out\crypto@XIII\else\def\crypto@VII@out{??}\fi\fi\fi\fi\fi\crypto@VII@out}\newcommand\crypto@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@VIII@out{\{"count": 310, "human": "310", "percent": "0.26\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@VIII@out{310}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@VIII@out{310}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@VIII@out{0.26\%}\else\def\crypto@VIII@out{??}\fi\fi\fi\fi\crypto@VIII@out}\newcommand\crypto@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@IX@out{\{"count": 3260, "human": "3.26K", "percent": "2.71\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@IX@out{3260}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@IX@out{3.26K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@IX@out{2.71\%}\else\def\crypto@IX@out{??}\fi\fi\fi\fi\crypto@IX@out}\newcommand\crypto@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@X@out{\{"count": 13519, "human": "13.5K", "percent": "11.22\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@X@out{13519}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@X@out{13.5K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@X@out{11.22\%}\else\def\crypto@X@out{??}\fi\fi\fi\fi\crypto@X@out}\newcommand\crypto@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XI@out{\{"count": 103423, "human": "103K", "percent": "85.82\%", "key\_sizes": \{"1536": \{"count": 1, "human": "1", "percent": "0.001\%"\}, "8192": \{"count": 147, "human": "147", "percent": "0.142\%"\}, "1024": \{"count": 148, "human": "148", "percent": "0.143\%"\}, "3072": \{"count": 2248, "human": "2.25K", "percent": "2.174\%"\}, "2048": \{"count": 49874, "human": "49.9K", "percent": "48.223\%"\}, "4096": \{"count": 51005, "human": "51K", "percent": "49.317\%"\}, "2560": \{"count": 0, "human": "0", "percent": "0.000\%"\}, "4608": \{"count": 0, "human": "0", "percent": "0.000\%"\}\}\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XI@out{103423}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XI@out{103K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XI@out{85.82\%}\else\ifnum\pdfstrcmp{#1}{key_sizes}=0\let\crypto@XI@out\crypto@XIV\else\def\crypto@XI@out{??}\fi\fi\fi\fi\fi\crypto@XI@out}\newcommand\crypto@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XII@out{\{"count": 0, "human": "0", "percent": "0.00\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XII@out{0}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XII@out{0}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XII@out{0.00\%}\else\def\crypto@XII@out{??}\fi\fi\fi\fi\crypto@XII@out}\newcommand\crypto@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XIII@out{\{"1536": \{"count": 20, "human": "20", "percent": "0.000\%"\}, "2560": \{"count": 142, "human": "142", "percent": "0.002\%"\}, "8192": \{"count": 374, "human": "374", "percent": "0.005\%"\}, "4608": \{"count": 402, "human": "402", "percent": "0.006\%"\}, "1024": \{"count": 19529, "human": "19.5K", "percent": "0.271\%"\}, "3072": \{"count": 999944, "human": "1M", "percent": "13.892\%"\}, "4096": \{"count": 2746911, "human": "2.75M", "percent": "38.162\%"\}, "2048": \{"count": 3430731, "human": "3.43M", "percent": "47.662\%"\}\}}\else\ifnum\pdfstrcmp{#1}{1536}=0\let\crypto@XIII@out\crypto@XV\else\ifnum\pdfstrcmp{#1}{2560}=0\let\crypto@XIII@out\crypto@XVI\else\ifnum\pdfstrcmp{#1}{8192}=0\let\crypto@XIII@out\crypto@XVII\else\ifnum\pdfstrcmp{#1}{4608}=0\let\crypto@XIII@out\crypto@XVIII\else\ifnum\pdfstrcmp{#1}{1024}=0\let\crypto@XIII@out\crypto@XIX\else\ifnum\pdfstrcmp{#1}{3072}=0\let\crypto@XIII@out\crypto@XX\else\ifnum\pdfstrcmp{#1}{4096}=0\let\crypto@XIII@out\crypto@XXI\else\ifnum\pdfstrcmp{#1}{2048}=0\let\crypto@XIII@out\crypto@XXII\else\def\crypto@XIII@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\crypto@XIII@out}\newcommand\crypto@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XIV@out{\{"1536": \{"count": 1, "human": "1", "percent": "0.001\%"\}, "8192": \{"count": 147, "human": "147", "percent": "0.142\%"\}, "1024": \{"count": 148, "human": "148", "percent": "0.143\%"\}, "3072": \{"count": 2248, "human": "2.25K", "percent": "2.174\%"\}, "2048": \{"count": 49874, "human": "49.9K", "percent": "48.223\%"\}, "4096": \{"count": 51005, "human": "51K", "percent": "49.317\%"\}, "2560": \{"count": 0, "human": "0", "percent": "0.000\%"\}, "4608": \{"count": 0, "human": "0", "percent": "0.000\%"\}\}}\else\ifnum\pdfstrcmp{#1}{1536}=0\let\crypto@XIV@out\crypto@XXIII\else\ifnum\pdfstrcmp{#1}{8192}=0\let\crypto@XIV@out\crypto@XXIV\else\ifnum\pdfstrcmp{#1}{1024}=0\let\crypto@XIV@out\crypto@XXV\else\ifnum\pdfstrcmp{#1}{3072}=0\let\crypto@XIV@out\crypto@XXVI\else\ifnum\pdfstrcmp{#1}{2048}=0\let\crypto@XIV@out\crypto@XXVII\else\ifnum\pdfstrcmp{#1}{4096}=0\let\crypto@XIV@out\crypto@XXVIII\else\ifnum\pdfstrcmp{#1}{2560}=0\let\crypto@XIV@out\crypto@XXIX\else\ifnum\pdfstrcmp{#1}{4608}=0\let\crypto@XIV@out\crypto@XXX\else\def\crypto@XIV@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\crypto@XIV@out}\newcommand\crypto@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XV@out{\{"count": 20, "human": "20", "percent": "0.000\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XV@out{20}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XV@out{20}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XV@out{0.000\%}\else\def\crypto@XV@out{??}\fi\fi\fi\fi\crypto@XV@out}\newcommand\crypto@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XVI@out{\{"count": 142, "human": "142", "percent": "0.002\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XVI@out{142}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XVI@out{142}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XVI@out{0.002\%}\else\def\crypto@XVI@out{??}\fi\fi\fi\fi\crypto@XVI@out}\newcommand\crypto@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XVII@out{\{"count": 374, "human": "374", "percent": "0.005\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XVII@out{374}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XVII@out{374}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XVII@out{0.005\%}\else\def\crypto@XVII@out{??}\fi\fi\fi\fi\crypto@XVII@out}\newcommand\crypto@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XVIII@out{\{"count": 402, "human": "402", "percent": "0.006\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XVIII@out{402}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XVIII@out{402}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XVIII@out{0.006\%}\else\def\crypto@XVIII@out{??}\fi\fi\fi\fi\crypto@XVIII@out}\newcommand\crypto@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XIX@out{\{"count": 19529, "human": "19.5K", "percent": "0.271\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XIX@out{19529}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XIX@out{19.5K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XIX@out{0.271\%}\else\def\crypto@XIX@out{??}\fi\fi\fi\fi\crypto@XIX@out}\newcommand\crypto@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XX@out{\{"count": 999944, "human": "1M", "percent": "13.892\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XX@out{999944}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XX@out{1M}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XX@out{13.892\%}\else\def\crypto@XX@out{??}\fi\fi\fi\fi\crypto@XX@out}\newcommand\crypto@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXI@out{\{"count": 2746911, "human": "2.75M", "percent": "38.162\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXI@out{2746911}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXI@out{2.75M}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXI@out{38.162\%}\else\def\crypto@XXI@out{??}\fi\fi\fi\fi\crypto@XXI@out}\newcommand\crypto@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXII@out{\{"count": 3430731, "human": "3.43M", "percent": "47.662\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXII@out{3430731}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXII@out{3.43M}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXII@out{47.662\%}\else\def\crypto@XXII@out{??}\fi\fi\fi\fi\crypto@XXII@out}\newcommand\crypto@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXIII@out{\{"count": 1, "human": "1", "percent": "0.001\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXIII@out{1}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXIII@out{1}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXIII@out{0.001\%}\else\def\crypto@XXIII@out{??}\fi\fi\fi\fi\crypto@XXIII@out}\newcommand\crypto@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXIV@out{\{"count": 147, "human": "147", "percent": "0.142\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXIV@out{147}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXIV@out{147}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXIV@out{0.142\%}\else\def\crypto@XXIV@out{??}\fi\fi\fi\fi\crypto@XXIV@out}\newcommand\crypto@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXV@out{\{"count": 148, "human": "148", "percent": "0.143\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXV@out{148}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXV@out{148}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXV@out{0.143\%}\else\def\crypto@XXV@out{??}\fi\fi\fi\fi\crypto@XXV@out}\newcommand\crypto@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXVI@out{\{"count": 2248, "human": "2.25K", "percent": "2.174\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXVI@out{2248}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXVI@out{2.25K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXVI@out{2.174\%}\else\def\crypto@XXVI@out{??}\fi\fi\fi\fi\crypto@XXVI@out}\newcommand\crypto@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXVII@out{\{"count": 49874, "human": "49.9K", "percent": "48.223\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXVII@out{49874}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXVII@out{49.9K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXVII@out{48.223\%}\else\def\crypto@XXVII@out{??}\fi\fi\fi\fi\crypto@XXVII@out}\newcommand\crypto@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXVIII@out{\{"count": 51005, "human": "51K", "percent": "49.317\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXVIII@out{51005}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXVIII@out{51K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXVIII@out{49.317\%}\else\def\crypto@XXVIII@out{??}\fi\fi\fi\fi\crypto@XXVIII@out}\newcommand\crypto@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXIX@out{\{"count": 0, "human": "0", "percent": "0.000\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXIX@out{0}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXIX@out{0}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXIX@out{0.000\%}\else\def\crypto@XXIX@out{??}\fi\fi\fi\fi\crypto@XXIX@out}\newcommand\crypto@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\crypto@XXX@out{\{"count": 0, "human": "0", "percent": "0.000\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\crypto@XXX@out{0}\else\ifnum\pdfstrcmp{#1}{human}=0\def\crypto@XXX@out{0}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\crypto@XXX@out{0.000\%}\else\def\crypto@XXX@out{??}\fi\fi\fi\fi\crypto@XXX@out}\makeatother

==> data/exp_keys.tex <==
\makeatletter\newcommand\expkeys[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@out{\{"maven": \{"total": 719084, "pub\_exp\_before": \{"count": 120467, "human": "120K", "percent": "16.8\%"\}, "pub\_exp\_after": \{"count": 598323, "human": "598K", "percent": "83.2\%"\}, "median\_remaining": "1.37", "upgrade\_paths": \{"total": \{"count": 8055, "human": "8.06K"\}, "upgradable": \{"count": 2150, "human": "2.15K", "percent": "26.7\%"\}\}\}, "pypi": \{"total": 19241, "pub\_exp\_before": \{"count": 2191, "human": "2.19K", "percent": "11.4\%"\}, "pub\_exp\_after": \{"count": 17049, "human": "17K", "percent": "88.6\%"\}, "median\_remaining": "1.93", "upgrade\_paths": \{"total": \{"count": 1082, "human": "1.08K"\}, "upgradable": \{"count": 87, "human": "87", "percent": "8.0\%"\}\}\}\}}\else\ifnum\pdfstrcmp{#1}{maven}=0\let\expkeys@out\expkeys@I\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\expkeys@out\expkeys@II\else\def\expkeys@out{??}\fi\fi\fi\expkeys@out}\newcommand\expkeys@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@I@out{\{"total": 719084, "pub\_exp\_before": \{"count": 120467, "human": "120K", "percent": "16.8\%"\}, "pub\_exp\_after": \{"count": 598323, "human": "598K", "percent": "83.2\%"\}, "median\_remaining": "1.37", "upgrade\_paths": \{"total": \{"count": 8055, "human": "8.06K"\}, "upgradable": \{"count": 2150, "human": "2.15K", "percent": "26.7\%"\}\}\}}\else\ifnum\pdfstrcmp{#1}{total}=0\def\expkeys@I@out{719084}\else\ifnum\pdfstrcmp{#1}{pub_exp_before}=0\let\expkeys@I@out\expkeys@III\else\ifnum\pdfstrcmp{#1}{pub_exp_after}=0\let\expkeys@I@out\expkeys@IV\else\ifnum\pdfstrcmp{#1}{median_remaining}=0\def\expkeys@I@out{1.37}\else\ifnum\pdfstrcmp{#1}{upgrade_paths}=0\let\expkeys@I@out\expkeys@V\else\def\expkeys@I@out{??}\fi\fi\fi\fi\fi\fi\expkeys@I@out}\newcommand\expkeys@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@II@out{\{"total": 19241, "pub\_exp\_before": \{"count": 2191, "human": "2.19K", "percent": "11.4\%"\}, "pub\_exp\_after": \{"count": 17049, "human": "17K", "percent": "88.6\%"\}, "median\_remaining": "1.93", "upgrade\_paths": \{"total": \{"count": 1082, "human": "1.08K"\}, "upgradable": \{"count": 87, "human": "87", "percent": "8.0\%"\}\}\}}\else\ifnum\pdfstrcmp{#1}{total}=0\def\expkeys@II@out{19241}\else\ifnum\pdfstrcmp{#1}{pub_exp_before}=0\let\expkeys@II@out\expkeys@VI\else\ifnum\pdfstrcmp{#1}{pub_exp_after}=0\let\expkeys@II@out\expkeys@VII\else\ifnum\pdfstrcmp{#1}{median_remaining}=0\def\expkeys@II@out{1.93}\else\ifnum\pdfstrcmp{#1}{upgrade_paths}=0\let\expkeys@II@out\expkeys@VIII\else\def\expkeys@II@out{??}\fi\fi\fi\fi\fi\fi\expkeys@II@out}\newcommand\expkeys@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@III@out{\{"count": 120467, "human": "120K", "percent": "16.8\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\expkeys@III@out{120467}\else\ifnum\pdfstrcmp{#1}{human}=0\def\expkeys@III@out{120K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\expkeys@III@out{16.8\%}\else\def\expkeys@III@out{??}\fi\fi\fi\fi\expkeys@III@out}\newcommand\expkeys@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@IV@out{\{"count": 598323, "human": "598K", "percent": "83.2\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\expkeys@IV@out{598323}\else\ifnum\pdfstrcmp{#1}{human}=0\def\expkeys@IV@out{598K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\expkeys@IV@out{83.2\%}\else\def\expkeys@IV@out{??}\fi\fi\fi\fi\expkeys@IV@out}\newcommand\expkeys@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@V@out{\{"total": \{"count": 8055, "human": "8.06K"\}, "upgradable": \{"count": 2150, "human": "2.15K", "percent": "26.7\%"\}\}}\else\ifnum\pdfstrcmp{#1}{total}=0\let\expkeys@V@out\expkeys@IX\else\ifnum\pdfstrcmp{#1}{upgradable}=0\let\expkeys@V@out\expkeys@X\else\def\expkeys@V@out{??}\fi\fi\fi\expkeys@V@out}\newcommand\expkeys@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@VI@out{\{"count": 2191, "human": "2.19K", "percent": "11.4\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\expkeys@VI@out{2191}\else\ifnum\pdfstrcmp{#1}{human}=0\def\expkeys@VI@out{2.19K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\expkeys@VI@out{11.4\%}\else\def\expkeys@VI@out{??}\fi\fi\fi\fi\expkeys@VI@out}\newcommand\expkeys@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@VII@out{\{"count": 17049, "human": "17K", "percent": "88.6\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\expkeys@VII@out{17049}\else\ifnum\pdfstrcmp{#1}{human}=0\def\expkeys@VII@out{17K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\expkeys@VII@out{88.6\%}\else\def\expkeys@VII@out{??}\fi\fi\fi\fi\expkeys@VII@out}\newcommand\expkeys@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@VIII@out{\{"total": \{"count": 1082, "human": "1.08K"\}, "upgradable": \{"count": 87, "human": "87", "percent": "8.0\%"\}\}}\else\ifnum\pdfstrcmp{#1}{total}=0\let\expkeys@VIII@out\expkeys@XI\else\ifnum\pdfstrcmp{#1}{upgradable}=0\let\expkeys@VIII@out\expkeys@XII\else\def\expkeys@VIII@out{??}\fi\fi\fi\expkeys@VIII@out}\newcommand\expkeys@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@IX@out{\{"count": 8055, "human": "8.06K"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\expkeys@IX@out{8055}\else\ifnum\pdfstrcmp{#1}{human}=0\def\expkeys@IX@out{8.06K}\else\def\expkeys@IX@out{??}\fi\fi\fi\expkeys@IX@out}\newcommand\expkeys@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@X@out{\{"count": 2150, "human": "2.15K", "percent": "26.7\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\expkeys@X@out{2150}\else\ifnum\pdfstrcmp{#1}{human}=0\def\expkeys@X@out{2.15K}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\expkeys@X@out{26.7\%}\else\def\expkeys@X@out{??}\fi\fi\fi\fi\expkeys@X@out}\newcommand\expkeys@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@XI@out{\{"count": 1082, "human": "1.08K"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\expkeys@XI@out{1082}\else\ifnum\pdfstrcmp{#1}{human}=0\def\expkeys@XI@out{1.08K}\else\def\expkeys@XI@out{??}\fi\fi\fi\expkeys@XI@out}\newcommand\expkeys@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\expkeys@XII@out{\{"count": 87, "human": "87", "percent": "8.0\%"\}}\else\ifnum\pdfstrcmp{#1}{count}=0\def\expkeys@XII@out{87}\else\ifnum\pdfstrcmp{#1}{human}=0\def\expkeys@XII@out{87}\else\ifnum\pdfstrcmp{#1}{percent}=0\def\expkeys@XII@out{8.0\%}\else\def\expkeys@XII@out{??}\fi\fi\fi\fi\expkeys@XII@out}\makeatother

==> data/metric.tex <==
\makeatletter\newcommand\metric[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\metric@out{\{"huggingface": \{"metric": 0.1510073432498588, "metric\_p": "15.10\%", "total": 2662807, "signed": 1850, "chance\_p": "0.07\%"\}, "docker": \{"metric": 0.8830335740453181, "metric\_p": "88.30\%", "total": 9517263, "signed": 234805, "chance\_p": "2.47\%"\}, "maven": \{"metric": 0.9600100962651568, "metric\_p": "96.00\%", "total": 7964488, "signed": 7497445, "chance\_p": "94.14\%"\}, "pypi": \{"metric": 0.4259861911253793, "metric\_p": "42.60\%", "total": 9677461, "signed": 120513, "chance\_p": "1.25\%"\}\}}\else\ifnum\pdfstrcmp{#1}{huggingface}=0\let\metric@out\metric@I\else\ifnum\pdfstrcmp{#1}{docker}=0\let\metric@out\metric@II\else\ifnum\pdfstrcmp{#1}{maven}=0\let\metric@out\metric@III\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\metric@out\metric@IV\else\def\metric@out{??}\fi\fi\fi\fi\fi\metric@out}\newcommand\metric@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\metric@I@out{\{"metric": 0.1510073432498588, "metric\_p": "15.10\%", "total": 2662807, "signed": 1850, "chance\_p": "0.07\%"\}}\else\ifnum\pdfstrcmp{#1}{metric}=0\def\metric@I@out{0.1510073432498588}\else\ifnum\pdfstrcmp{#1}{metric_p}=0\def\metric@I@out{15.10\%}\else\ifnum\pdfstrcmp{#1}{total}=0\def\metric@I@out{2662807}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\metric@I@out{1850}\else\ifnum\pdfstrcmp{#1}{chance_p}=0\def\metric@I@out{0.07\%}\else\def\metric@I@out{??}\fi\fi\fi\fi\fi\fi\metric@I@out}\newcommand\metric@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\metric@II@out{\{"metric": 0.8830335740453181, "metric\_p": "88.30\%", "total": 9517263, "signed": 234805, "chance\_p": "2.47\%"\}}\else\ifnum\pdfstrcmp{#1}{metric}=0\def\metric@II@out{0.8830335740453181}\else\ifnum\pdfstrcmp{#1}{metric_p}=0\def\metric@II@out{88.30\%}\else\ifnum\pdfstrcmp{#1}{total}=0\def\metric@II@out{9517263}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\metric@II@out{234805}\else\ifnum\pdfstrcmp{#1}{chance_p}=0\def\metric@II@out{2.47\%}\else\def\metric@II@out{??}\fi\fi\fi\fi\fi\fi\metric@II@out}\newcommand\metric@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\metric@III@out{\{"metric": 0.9600100962651568, "metric\_p": "96.00\%", "total": 7964488, "signed": 7497445, "chance\_p": "94.14\%"\}}\else\ifnum\pdfstrcmp{#1}{metric}=0\def\metric@III@out{0.9600100962651568}\else\ifnum\pdfstrcmp{#1}{metric_p}=0\def\metric@III@out{96.00\%}\else\ifnum\pdfstrcmp{#1}{total}=0\def\metric@III@out{7964488}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\metric@III@out{7497445}\else\ifnum\pdfstrcmp{#1}{chance_p}=0\def\metric@III@out{94.14\%}\else\def\metric@III@out{??}\fi\fi\fi\fi\fi\fi\metric@III@out}\newcommand\metric@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\metric@IV@out{\{"metric": 0.4259861911253793, "metric\_p": "42.60\%", "total": 9677461, "signed": 120513, "chance\_p": "1.25\%"\}}\else\ifnum\pdfstrcmp{#1}{metric}=0\def\metric@IV@out{0.4259861911253793}\else\ifnum\pdfstrcmp{#1}{metric_p}=0\def\metric@IV@out{42.60\%}\else\ifnum\pdfstrcmp{#1}{total}=0\def\metric@IV@out{9677461}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\metric@IV@out{120513}\else\ifnum\pdfstrcmp{#1}{chance_p}=0\def\metric@IV@out{1.25\%}\else\def\metric@IV@out{??}\fi\fi\fi\fi\fi\fi\metric@IV@out}\makeatother

==> data/stats.tex <==
\makeatletter\newcommand\stats[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@out{\{"anova": \{"f": "116135.82", "p": "0.000"\}, "tukey": \{"huggingface": \{"huggingface": \{"statistic": "0.00", "p": "1.000"\}, "docker": \{"statistic": "91.14", "p": "0.000"\}, "maven": \{"statistic": "90.03", "p": "0.000"\}, "pypi": \{"statistic": "91.65", "p": "0.000"\}\}, "docker": \{"huggingface": \{"statistic": "{-}91.14", "p": "0.000"\}, "docker": \{"statistic": "0.00", "p": "1.000"\}, "maven": \{"statistic": "{-}1.11", "p": "0.000"\}, "pypi": \{"statistic": "0.51", "p": "0.099"\}\}, "maven": \{"huggingface": \{"statistic": "{-}90.03", "p": "0.000"\}, "docker": \{"statistic": "1.11", "p": "0.000"\}, "maven": \{"statistic": "0.00", "p": "1.000"\}, "pypi": \{"statistic": "1.62", "p": "0.000"\}\}, "pypi": \{"huggingface": \{"statistic": "{-}91.65", "p": "0.000"\}, "docker": \{"statistic": "{-}0.51", "p": "0.099"\}, "maven": \{"statistic": "{-}1.62", "p": "0.000"\}, "pypi": \{"statistic": "0.00", "p": "1.000"\}\}\}, "ttests": \{"pypi\_deemp": \{"pypi": \{"t\_statistic": 4.31074916339165, "p\_value": 1.0528800972503641e{-}05, "effect\_size": "0.228", "before": \{"mean": 5.07728279552548, "std": 3.341110495164511\}, "after": \{"mean": 3.762475440194618, "std": 2.362671322667053\}, "adj\_p": "0.000"\}, "maven": \{"t\_statistic": 1.6095209739825587, "p\_value": 0.054191933477561106, "effect\_size": "0.085", "before": \{"mean": 94.80552152298739, "std": 6.60344205728319\}, "after": \{"mean": 93.57771768771765, "std": 7.819238599420711\}, "adj\_p": "0.081"\}, "docker": \{"t\_statistic": 2.811217881729063, "p\_value": 0.0026035239065010825, "effect\_size": "0.149", "before": \{"mean": 1.214229900214069, "std": 2.443644732339022\}, "after": \{"mean": 0.6652851932595292, "std": 0.9444693288506714\}, "adj\_p": "0.005"\}\}, "docker\_update": \{"pypi": \{"t\_statistic": 1.8984972917971132, "p\_value": 0.9707827344233013, "effect\_size": "0.100", "before": \{"mean": 2.2961581361167376, "std": 1.9902588271563522\}, "after": \{"mean": 1.938145082278047, "std": 1.5620197624637286\}, "adj\_p": "0.971"\}, "maven": \{"t\_statistic": 1.2477265754687297, "p\_value": 0.8935266393500214, "effect\_size": "0.066", "before": \{"mean": 94.14208165393968, "std": 8.120872618703146\}, "after": \{"mean": 92.98239253273496, "std": 9.462904856958765\}, "adj\_p": "0.971"\}, "docker": \{"t\_statistic": {-}7.419901479563398, "p\_value": 4.299451618877173e{-}13, "effect\_size": "0.392", "before": \{"mean": 1.8307136568351885, "std": 2.652931530658601\}, "after": \{"mean": 5.229468421866609, "std": 5.5433969553392135\}, "adj\_p": "0.000"\}\}, "docker\_hack": \{"pypi": \{"t\_statistic": 3.2141269933972536, "p\_value": 0.9992863507506341, "effect\_size": "0.170", "before": \{"mean": 2.8275318786245656, "std": 2.6866561167896887\}, "after": \{"mean": 2.0505510997680045, "std": 1.8167823562978915\}, "adj\_p": "0.999"\}, "maven": \{"t\_statistic": 2.208820810501289, "p\_value": 0.9860899998462503, "effect\_size": "0.117", "before": \{"mean": 95.2155606928716, "std": 6.823432642887064\}, "after": \{"mean": 93.49265301745906, "std": 7.934497826624769\}, "adj\_p": "0.999"\}, "docker": \{"t\_statistic": {-}2.44411561644384, "p\_value": 0.007501344529292149, "effect\_size": "0.129", "before": \{"mean": 1.2868743196879324, "std": 1.9110147811740117\}, "after": \{"mean": 1.9024102977600428, "std": 2.786503040500623\}, "adj\_p": "0.021"\}\}, "solarwinds": \{"pypi": \{"t\_statistic": 0.2924723002247588, "p\_value": 0.6149525171398281, "effect\_size": "0.015", "before": \{"mean": 0.867865724112823, "std": 0.9000931203616069\}, "after": \{"mean": 0.8417458923621104, "std": 0.7908644022261112\}, "adj\_p": "0.922"\}, "maven": \{"t\_statistic": {-}2.7193347331582762, "p\_value": 0.0034300346672920933, "effect\_size": "0.144", "before": \{"mean": 94.82981224587567, "std": 7.186417040483126\}, "after": \{"mean": 96.653111411263, "std": 5.410798812779476\}, "adj\_p": "0.021"\}, "docker": \{"t\_statistic": {-}2.3166357467499923, "p\_value": 0.01054375099817995, "effect\_size": "0.122", "before": \{"mean": 9.477527730103349, "std": 3.7853584897791857\}, "after": \{"mean": 10.42505917928366, "std": 3.9728307838983334\}, "adj\_p": "0.021"\}\}\}\}}\else\ifnum\pdfstrcmp{#1}{anova}=0\let\stats@out\stats@I\else\ifnum\pdfstrcmp{#1}{tukey}=0\let\stats@out\stats@II\else\ifnum\pdfstrcmp{#1}{ttests}=0\let\stats@out\stats@III\else\def\stats@out{??}\fi\fi\fi\fi\stats@out}\newcommand\stats@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@I@out{\{"f": "116135.82", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{f}=0\def\stats@I@out{116135.82}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@I@out{0.000}\else\def\stats@I@out{??}\fi\fi\fi\stats@I@out}\newcommand\stats@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@II@out{\{"huggingface": \{"huggingface": \{"statistic": "0.00", "p": "1.000"\}, "docker": \{"statistic": "91.14", "p": "0.000"\}, "maven": \{"statistic": "90.03", "p": "0.000"\}, "pypi": \{"statistic": "91.65", "p": "0.000"\}\}, "docker": \{"huggingface": \{"statistic": "{-}91.14", "p": "0.000"\}, "docker": \{"statistic": "0.00", "p": "1.000"\}, "maven": \{"statistic": "{-}1.11", "p": "0.000"\}, "pypi": \{"statistic": "0.51", "p": "0.099"\}\}, "maven": \{"huggingface": \{"statistic": "{-}90.03", "p": "0.000"\}, "docker": \{"statistic": "1.11", "p": "0.000"\}, "maven": \{"statistic": "0.00", "p": "1.000"\}, "pypi": \{"statistic": "1.62", "p": "0.000"\}\}, "pypi": \{"huggingface": \{"statistic": "{-}91.65", "p": "0.000"\}, "docker": \{"statistic": "{-}0.51", "p": "0.099"\}, "maven": \{"statistic": "{-}1.62", "p": "0.000"\}, "pypi": \{"statistic": "0.00", "p": "1.000"\}\}\}}\else\ifnum\pdfstrcmp{#1}{huggingface}=0\let\stats@II@out\stats@IV\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@II@out\stats@V\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@II@out\stats@VI\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@II@out\stats@VII\else\def\stats@II@out{??}\fi\fi\fi\fi\fi\stats@II@out}\newcommand\stats@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@III@out{\{"pypi\_deemp": \{"pypi": \{"t\_statistic": 4.31074916339165, "p\_value": 1.0528800972503641e{-}05, "effect\_size": "0.228", "before": \{"mean": 5.07728279552548, "std": 3.341110495164511\}, "after": \{"mean": 3.762475440194618, "std": 2.362671322667053\}, "adj\_p": "0.000"\}, "maven": \{"t\_statistic": 1.6095209739825587, "p\_value": 0.054191933477561106, "effect\_size": "0.085", "before": \{"mean": 94.80552152298739, "std": 6.60344205728319\}, "after": \{"mean": 93.57771768771765, "std": 7.819238599420711\}, "adj\_p": "0.081"\}, "docker": \{"t\_statistic": 2.811217881729063, "p\_value": 0.0026035239065010825, "effect\_size": "0.149", "before": \{"mean": 1.214229900214069, "std": 2.443644732339022\}, "after": \{"mean": 0.6652851932595292, "std": 0.9444693288506714\}, "adj\_p": "0.005"\}\}, "docker\_update": \{"pypi": \{"t\_statistic": 1.8984972917971132, "p\_value": 0.9707827344233013, "effect\_size": "0.100", "before": \{"mean": 2.2961581361167376, "std": 1.9902588271563522\}, "after": \{"mean": 1.938145082278047, "std": 1.5620197624637286\}, "adj\_p": "0.971"\}, "maven": \{"t\_statistic": 1.2477265754687297, "p\_value": 0.8935266393500214, "effect\_size": "0.066", "before": \{"mean": 94.14208165393968, "std": 8.120872618703146\}, "after": \{"mean": 92.98239253273496, "std": 9.462904856958765\}, "adj\_p": "0.971"\}, "docker": \{"t\_statistic": {-}7.419901479563398, "p\_value": 4.299451618877173e{-}13, "effect\_size": "0.392", "before": \{"mean": 1.8307136568351885, "std": 2.652931530658601\}, "after": \{"mean": 5.229468421866609, "std": 5.5433969553392135\}, "adj\_p": "0.000"\}\}, "docker\_hack": \{"pypi": \{"t\_statistic": 3.2141269933972536, "p\_value": 0.9992863507506341, "effect\_size": "0.170", "before": \{"mean": 2.8275318786245656, "std": 2.6866561167896887\}, "after": \{"mean": 2.0505510997680045, "std": 1.8167823562978915\}, "adj\_p": "0.999"\}, "maven": \{"t\_statistic": 2.208820810501289, "p\_value": 0.9860899998462503, "effect\_size": "0.117", "before": \{"mean": 95.2155606928716, "std": 6.823432642887064\}, "after": \{"mean": 93.49265301745906, "std": 7.934497826624769\}, "adj\_p": "0.999"\}, "docker": \{"t\_statistic": {-}2.44411561644384, "p\_value": 0.007501344529292149, "effect\_size": "0.129", "before": \{"mean": 1.2868743196879324, "std": 1.9110147811740117\}, "after": \{"mean": 1.9024102977600428, "std": 2.786503040500623\}, "adj\_p": "0.021"\}\}, "solarwinds": \{"pypi": \{"t\_statistic": 0.2924723002247588, "p\_value": 0.6149525171398281, "effect\_size": "0.015", "before": \{"mean": 0.867865724112823, "std": 0.9000931203616069\}, "after": \{"mean": 0.8417458923621104, "std": 0.7908644022261112\}, "adj\_p": "0.922"\}, "maven": \{"t\_statistic": {-}2.7193347331582762, "p\_value": 0.0034300346672920933, "effect\_size": "0.144", "before": \{"mean": 94.82981224587567, "std": 7.186417040483126\}, "after": \{"mean": 96.653111411263, "std": 5.410798812779476\}, "adj\_p": "0.021"\}, "docker": \{"t\_statistic": {-}2.3166357467499923, "p\_value": 0.01054375099817995, "effect\_size": "0.122", "before": \{"mean": 9.477527730103349, "std": 3.7853584897791857\}, "after": \{"mean": 10.42505917928366, "std": 3.9728307838983334\}, "adj\_p": "0.021"\}\}\}}\else\ifnum\pdfstrcmp{#1}{pypi_deemp}=0\let\stats@III@out\stats@VIII\else\ifnum\pdfstrcmp{#1}{docker_update}=0\let\stats@III@out\stats@IX\else\ifnum\pdfstrcmp{#1}{docker_hack}=0\let\stats@III@out\stats@X\else\ifnum\pdfstrcmp{#1}{solarwinds}=0\let\stats@III@out\stats@XI\else\def\stats@III@out{??}\fi\fi\fi\fi\fi\stats@III@out}\newcommand\stats@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@IV@out{\{"huggingface": \{"statistic": "0.00", "p": "1.000"\}, "docker": \{"statistic": "91.14", "p": "0.000"\}, "maven": \{"statistic": "90.03", "p": "0.000"\}, "pypi": \{"statistic": "91.65", "p": "0.000"\}\}}\else\ifnum\pdfstrcmp{#1}{huggingface}=0\let\stats@IV@out\stats@XII\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@IV@out\stats@XIII\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@IV@out\stats@XIV\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@IV@out\stats@XV\else\def\stats@IV@out{??}\fi\fi\fi\fi\fi\stats@IV@out}\newcommand\stats@V[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@V@out{\{"huggingface": \{"statistic": "{-}91.14", "p": "0.000"\}, "docker": \{"statistic": "0.00", "p": "1.000"\}, "maven": \{"statistic": "{-}1.11", "p": "0.000"\}, "pypi": \{"statistic": "0.51", "p": "0.099"\}\}}\else\ifnum\pdfstrcmp{#1}{huggingface}=0\let\stats@V@out\stats@XVI\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@V@out\stats@XVII\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@V@out\stats@XVIII\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@V@out\stats@XIX\else\def\stats@V@out{??}\fi\fi\fi\fi\fi\stats@V@out}\newcommand\stats@VI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@VI@out{\{"huggingface": \{"statistic": "{-}90.03", "p": "0.000"\}, "docker": \{"statistic": "1.11", "p": "0.000"\}, "maven": \{"statistic": "0.00", "p": "1.000"\}, "pypi": \{"statistic": "1.62", "p": "0.000"\}\}}\else\ifnum\pdfstrcmp{#1}{huggingface}=0\let\stats@VI@out\stats@XX\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@VI@out\stats@XXI\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@VI@out\stats@XXII\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@VI@out\stats@XXIII\else\def\stats@VI@out{??}\fi\fi\fi\fi\fi\stats@VI@out}\newcommand\stats@VII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@VII@out{\{"huggingface": \{"statistic": "{-}91.65", "p": "0.000"\}, "docker": \{"statistic": "{-}0.51", "p": "0.099"\}, "maven": \{"statistic": "{-}1.62", "p": "0.000"\}, "pypi": \{"statistic": "0.00", "p": "1.000"\}\}}\else\ifnum\pdfstrcmp{#1}{huggingface}=0\let\stats@VII@out\stats@XXIV\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@VII@out\stats@XXV\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@VII@out\stats@XXVI\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@VII@out\stats@XXVII\else\def\stats@VII@out{??}\fi\fi\fi\fi\fi\stats@VII@out}\newcommand\stats@VIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@VIII@out{\{"pypi": \{"t\_statistic": 4.31074916339165, "p\_value": 1.0528800972503641e{-}05, "effect\_size": "0.228", "before": \{"mean": 5.07728279552548, "std": 3.341110495164511\}, "after": \{"mean": 3.762475440194618, "std": 2.362671322667053\}, "adj\_p": "0.000"\}, "maven": \{"t\_statistic": 1.6095209739825587, "p\_value": 0.054191933477561106, "effect\_size": "0.085", "before": \{"mean": 94.80552152298739, "std": 6.60344205728319\}, "after": \{"mean": 93.57771768771765, "std": 7.819238599420711\}, "adj\_p": "0.081"\}, "docker": \{"t\_statistic": 2.811217881729063, "p\_value": 0.0026035239065010825, "effect\_size": "0.149", "before": \{"mean": 1.214229900214069, "std": 2.443644732339022\}, "after": \{"mean": 0.6652851932595292, "std": 0.9444693288506714\}, "adj\_p": "0.005"\}\}}\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@VIII@out\stats@XXVIII\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@VIII@out\stats@XXIX\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@VIII@out\stats@XXX\else\def\stats@VIII@out{??}\fi\fi\fi\fi\stats@VIII@out}\newcommand\stats@IX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@IX@out{\{"pypi": \{"t\_statistic": 1.8984972917971132, "p\_value": 0.9707827344233013, "effect\_size": "0.100", "before": \{"mean": 2.2961581361167376, "std": 1.9902588271563522\}, "after": \{"mean": 1.938145082278047, "std": 1.5620197624637286\}, "adj\_p": "0.971"\}, "maven": \{"t\_statistic": 1.2477265754687297, "p\_value": 0.8935266393500214, "effect\_size": "0.066", "before": \{"mean": 94.14208165393968, "std": 8.120872618703146\}, "after": \{"mean": 92.98239253273496, "std": 9.462904856958765\}, "adj\_p": "0.971"\}, "docker": \{"t\_statistic": {-}7.419901479563398, "p\_value": 4.299451618877173e{-}13, "effect\_size": "0.392", "before": \{"mean": 1.8307136568351885, "std": 2.652931530658601\}, "after": \{"mean": 5.229468421866609, "std": 5.5433969553392135\}, "adj\_p": "0.000"\}\}}\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@IX@out\stats@XXXI\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@IX@out\stats@XXXII\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@IX@out\stats@XXXIII\else\def\stats@IX@out{??}\fi\fi\fi\fi\stats@IX@out}\newcommand\stats@X[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@X@out{\{"pypi": \{"t\_statistic": 3.2141269933972536, "p\_value": 0.9992863507506341, "effect\_size": "0.170", "before": \{"mean": 2.8275318786245656, "std": 2.6866561167896887\}, "after": \{"mean": 2.0505510997680045, "std": 1.8167823562978915\}, "adj\_p": "0.999"\}, "maven": \{"t\_statistic": 2.208820810501289, "p\_value": 0.9860899998462503, "effect\_size": "0.117", "before": \{"mean": 95.2155606928716, "std": 6.823432642887064\}, "after": \{"mean": 93.49265301745906, "std": 7.934497826624769\}, "adj\_p": "0.999"\}, "docker": \{"t\_statistic": {-}2.44411561644384, "p\_value": 0.007501344529292149, "effect\_size": "0.129", "before": \{"mean": 1.2868743196879324, "std": 1.9110147811740117\}, "after": \{"mean": 1.9024102977600428, "std": 2.786503040500623\}, "adj\_p": "0.021"\}\}}\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@X@out\stats@XXXIV\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@X@out\stats@XXXV\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@X@out\stats@XXXVI\else\def\stats@X@out{??}\fi\fi\fi\fi\stats@X@out}\newcommand\stats@XI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XI@out{\{"pypi": \{"t\_statistic": 0.2924723002247588, "p\_value": 0.6149525171398281, "effect\_size": "0.015", "before": \{"mean": 0.867865724112823, "std": 0.9000931203616069\}, "after": \{"mean": 0.8417458923621104, "std": 0.7908644022261112\}, "adj\_p": "0.922"\}, "maven": \{"t\_statistic": {-}2.7193347331582762, "p\_value": 0.0034300346672920933, "effect\_size": "0.144", "before": \{"mean": 94.82981224587567, "std": 7.186417040483126\}, "after": \{"mean": 96.653111411263, "std": 5.410798812779476\}, "adj\_p": "0.021"\}, "docker": \{"t\_statistic": {-}2.3166357467499923, "p\_value": 0.01054375099817995, "effect\_size": "0.122", "before": \{"mean": 9.477527730103349, "std": 3.7853584897791857\}, "after": \{"mean": 10.42505917928366, "std": 3.9728307838983334\}, "adj\_p": "0.021"\}\}}\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\stats@XI@out\stats@XXXVII\else\ifnum\pdfstrcmp{#1}{maven}=0\let\stats@XI@out\stats@XXXVIII\else\ifnum\pdfstrcmp{#1}{docker}=0\let\stats@XI@out\stats@XXXIX\else\def\stats@XI@out{??}\fi\fi\fi\fi\stats@XI@out}\newcommand\stats@XII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XII@out{\{"statistic": "0.00", "p": "1.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XII@out{0.00}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XII@out{1.000}\else\def\stats@XII@out{??}\fi\fi\fi\stats@XII@out}\newcommand\stats@XIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XIII@out{\{"statistic": "91.14", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XIII@out{91.14}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XIII@out{0.000}\else\def\stats@XIII@out{??}\fi\fi\fi\stats@XIII@out}\newcommand\stats@XIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XIV@out{\{"statistic": "90.03", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XIV@out{90.03}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XIV@out{0.000}\else\def\stats@XIV@out{??}\fi\fi\fi\stats@XIV@out}\newcommand\stats@XV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XV@out{\{"statistic": "91.65", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XV@out{91.65}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XV@out{0.000}\else\def\stats@XV@out{??}\fi\fi\fi\stats@XV@out}\newcommand\stats@XVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XVI@out{\{"statistic": "{-}91.14", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XVI@out{{-}91.14}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XVI@out{0.000}\else\def\stats@XVI@out{??}\fi\fi\fi\stats@XVI@out}\newcommand\stats@XVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XVII@out{\{"statistic": "0.00", "p": "1.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XVII@out{0.00}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XVII@out{1.000}\else\def\stats@XVII@out{??}\fi\fi\fi\stats@XVII@out}\newcommand\stats@XVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XVIII@out{\{"statistic": "{-}1.11", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XVIII@out{{-}1.11}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XVIII@out{0.000}\else\def\stats@XVIII@out{??}\fi\fi\fi\stats@XVIII@out}\newcommand\stats@XIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XIX@out{\{"statistic": "0.51", "p": "0.099"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XIX@out{0.51}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XIX@out{0.099}\else\def\stats@XIX@out{??}\fi\fi\fi\stats@XIX@out}\newcommand\stats@XX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XX@out{\{"statistic": "{-}90.03", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XX@out{{-}90.03}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XX@out{0.000}\else\def\stats@XX@out{??}\fi\fi\fi\stats@XX@out}\newcommand\stats@XXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXI@out{\{"statistic": "1.11", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XXI@out{1.11}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XXI@out{0.000}\else\def\stats@XXI@out{??}\fi\fi\fi\stats@XXI@out}\newcommand\stats@XXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXII@out{\{"statistic": "0.00", "p": "1.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XXII@out{0.00}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XXII@out{1.000}\else\def\stats@XXII@out{??}\fi\fi\fi\stats@XXII@out}\newcommand\stats@XXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXIII@out{\{"statistic": "1.62", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XXIII@out{1.62}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XXIII@out{0.000}\else\def\stats@XXIII@out{??}\fi\fi\fi\stats@XXIII@out}\newcommand\stats@XXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXIV@out{\{"statistic": "{-}91.65", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XXIV@out{{-}91.65}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XXIV@out{0.000}\else\def\stats@XXIV@out{??}\fi\fi\fi\stats@XXIV@out}\newcommand\stats@XXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXV@out{\{"statistic": "{-}0.51", "p": "0.099"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XXV@out{{-}0.51}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XXV@out{0.099}\else\def\stats@XXV@out{??}\fi\fi\fi\stats@XXV@out}\newcommand\stats@XXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXVI@out{\{"statistic": "{-}1.62", "p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XXVI@out{{-}1.62}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XXVI@out{0.000}\else\def\stats@XXVI@out{??}\fi\fi\fi\stats@XXVI@out}\newcommand\stats@XXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXVII@out{\{"statistic": "0.00", "p": "1.000"\}}\else\ifnum\pdfstrcmp{#1}{statistic}=0\def\stats@XXVII@out{0.00}\else\ifnum\pdfstrcmp{#1}{p}=0\def\stats@XXVII@out{1.000}\else\def\stats@XXVII@out{??}\fi\fi\fi\stats@XXVII@out}\newcommand\stats@XXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXVIII@out{\{"t\_statistic": 4.31074916339165, "p\_value": 1.0528800972503641e{-}05, "effect\_size": "0.228", "before": \{"mean": 5.07728279552548, "std": 3.341110495164511\}, "after": \{"mean": 3.762475440194618, "std": 2.362671322667053\}, "adj\_p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXVIII@out{4.31074916339165}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXVIII@out{1.0528800972503641e{-}05}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXVIII@out{0.228}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXVIII@out\stats@XL\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXVIII@out\stats@XLI\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXVIII@out{0.000}\else\def\stats@XXVIII@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXVIII@out}\newcommand\stats@XXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXIX@out{\{"t\_statistic": 1.6095209739825587, "p\_value": 0.054191933477561106, "effect\_size": "0.085", "before": \{"mean": 94.80552152298739, "std": 6.60344205728319\}, "after": \{"mean": 93.57771768771765, "std": 7.819238599420711\}, "adj\_p": "0.081"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXIX@out{1.6095209739825587}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXIX@out{0.054191933477561106}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXIX@out{0.085}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXIX@out\stats@XLII\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXIX@out\stats@XLIII\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXIX@out{0.081}\else\def\stats@XXIX@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXIX@out}\newcommand\stats@XXX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXX@out{\{"t\_statistic": 2.811217881729063, "p\_value": 0.0026035239065010825, "effect\_size": "0.149", "before": \{"mean": 1.214229900214069, "std": 2.443644732339022\}, "after": \{"mean": 0.6652851932595292, "std": 0.9444693288506714\}, "adj\_p": "0.005"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXX@out{2.811217881729063}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXX@out{0.0026035239065010825}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXX@out{0.149}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXX@out\stats@XLIV\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXX@out\stats@XLV\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXX@out{0.005}\else\def\stats@XXX@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXX@out}\newcommand\stats@XXXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXI@out{\{"t\_statistic": 1.8984972917971132, "p\_value": 0.9707827344233013, "effect\_size": "0.100", "before": \{"mean": 2.2961581361167376, "std": 1.9902588271563522\}, "after": \{"mean": 1.938145082278047, "std": 1.5620197624637286\}, "adj\_p": "0.971"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXI@out{1.8984972917971132}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXI@out{0.9707827344233013}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXI@out{0.100}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXI@out\stats@XLVI\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXI@out\stats@XLVII\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXI@out{0.971}\else\def\stats@XXXI@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXI@out}\newcommand\stats@XXXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXII@out{\{"t\_statistic": 1.2477265754687297, "p\_value": 0.8935266393500214, "effect\_size": "0.066", "before": \{"mean": 94.14208165393968, "std": 8.120872618703146\}, "after": \{"mean": 92.98239253273496, "std": 9.462904856958765\}, "adj\_p": "0.971"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXII@out{1.2477265754687297}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXII@out{0.8935266393500214}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXII@out{0.066}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXII@out\stats@XLVIII\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXII@out\stats@XLIX\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXII@out{0.971}\else\def\stats@XXXII@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXII@out}\newcommand\stats@XXXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXIII@out{\{"t\_statistic": {-}7.419901479563398, "p\_value": 4.299451618877173e{-}13, "effect\_size": "0.392", "before": \{"mean": 1.8307136568351885, "std": 2.652931530658601\}, "after": \{"mean": 5.229468421866609, "std": 5.5433969553392135\}, "adj\_p": "0.000"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXIII@out{{-}7.419901479563398}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXIII@out{4.299451618877173e{-}13}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXIII@out{0.392}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXIII@out\stats@L\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXIII@out\stats@LI\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXIII@out{0.000}\else\def\stats@XXXIII@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXIII@out}\newcommand\stats@XXXIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXIV@out{\{"t\_statistic": 3.2141269933972536, "p\_value": 0.9992863507506341, "effect\_size": "0.170", "before": \{"mean": 2.8275318786245656, "std": 2.6866561167896887\}, "after": \{"mean": 2.0505510997680045, "std": 1.8167823562978915\}, "adj\_p": "0.999"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXIV@out{3.2141269933972536}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXIV@out{0.9992863507506341}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXIV@out{0.170}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXIV@out\stats@LII\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXIV@out\stats@LIII\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXIV@out{0.999}\else\def\stats@XXXIV@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXIV@out}\newcommand\stats@XXXV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXV@out{\{"t\_statistic": 2.208820810501289, "p\_value": 0.9860899998462503, "effect\_size": "0.117", "before": \{"mean": 95.2155606928716, "std": 6.823432642887064\}, "after": \{"mean": 93.49265301745906, "std": 7.934497826624769\}, "adj\_p": "0.999"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXV@out{2.208820810501289}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXV@out{0.9860899998462503}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXV@out{0.117}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXV@out\stats@LIV\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXV@out\stats@LV\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXV@out{0.999}\else\def\stats@XXXV@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXV@out}\newcommand\stats@XXXVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXVI@out{\{"t\_statistic": {-}2.44411561644384, "p\_value": 0.007501344529292149, "effect\_size": "0.129", "before": \{"mean": 1.2868743196879324, "std": 1.9110147811740117\}, "after": \{"mean": 1.9024102977600428, "std": 2.786503040500623\}, "adj\_p": "0.021"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXVI@out{{-}2.44411561644384}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXVI@out{0.007501344529292149}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXVI@out{0.129}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXVI@out\stats@LVI\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXVI@out\stats@LVII\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXVI@out{0.021}\else\def\stats@XXXVI@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXVI@out}\newcommand\stats@XXXVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXVII@out{\{"t\_statistic": 0.2924723002247588, "p\_value": 0.6149525171398281, "effect\_size": "0.015", "before": \{"mean": 0.867865724112823, "std": 0.9000931203616069\}, "after": \{"mean": 0.8417458923621104, "std": 0.7908644022261112\}, "adj\_p": "0.922"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXVII@out{0.2924723002247588}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXVII@out{0.6149525171398281}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXVII@out{0.015}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXVII@out\stats@LVIII\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXVII@out\stats@LIX\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXVII@out{0.922}\else\def\stats@XXXVII@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXVII@out}\newcommand\stats@XXXVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXVIII@out{\{"t\_statistic": {-}2.7193347331582762, "p\_value": 0.0034300346672920933, "effect\_size": "0.144", "before": \{"mean": 94.82981224587567, "std": 7.186417040483126\}, "after": \{"mean": 96.653111411263, "std": 5.410798812779476\}, "adj\_p": "0.021"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXVIII@out{{-}2.7193347331582762}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXVIII@out{0.0034300346672920933}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXVIII@out{0.144}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXVIII@out\stats@LX\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXVIII@out\stats@LXI\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXVIII@out{0.021}\else\def\stats@XXXVIII@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXVIII@out}\newcommand\stats@XXXIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XXXIX@out{\{"t\_statistic": {-}2.3166357467499923, "p\_value": 0.01054375099817995, "effect\_size": "0.122", "before": \{"mean": 9.477527730103349, "std": 3.7853584897791857\}, "after": \{"mean": 10.42505917928366, "std": 3.9728307838983334\}, "adj\_p": "0.021"\}}\else\ifnum\pdfstrcmp{#1}{t_statistic}=0\def\stats@XXXIX@out{{-}2.3166357467499923}\else\ifnum\pdfstrcmp{#1}{p_value}=0\def\stats@XXXIX@out{0.01054375099817995}\else\ifnum\pdfstrcmp{#1}{effect_size}=0\def\stats@XXXIX@out{0.122}\else\ifnum\pdfstrcmp{#1}{before}=0\let\stats@XXXIX@out\stats@LXII\else\ifnum\pdfstrcmp{#1}{after}=0\let\stats@XXXIX@out\stats@LXIII\else\ifnum\pdfstrcmp{#1}{adj_p}=0\def\stats@XXXIX@out{0.021}\else\def\stats@XXXIX@out{??}\fi\fi\fi\fi\fi\fi\fi\stats@XXXIX@out}\newcommand\stats@XL[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XL@out{\{"mean": 5.07728279552548, "std": 3.341110495164511\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XL@out{5.07728279552548}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XL@out{3.341110495164511}\else\def\stats@XL@out{??}\fi\fi\fi\stats@XL@out}\newcommand\stats@XLI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLI@out{\{"mean": 3.762475440194618, "std": 2.362671322667053\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLI@out{3.762475440194618}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLI@out{2.362671322667053}\else\def\stats@XLI@out{??}\fi\fi\fi\stats@XLI@out}\newcommand\stats@XLII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLII@out{\{"mean": 94.80552152298739, "std": 6.60344205728319\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLII@out{94.80552152298739}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLII@out{6.60344205728319}\else\def\stats@XLII@out{??}\fi\fi\fi\stats@XLII@out}\newcommand\stats@XLIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLIII@out{\{"mean": 93.57771768771765, "std": 7.819238599420711\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLIII@out{93.57771768771765}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLIII@out{7.819238599420711}\else\def\stats@XLIII@out{??}\fi\fi\fi\stats@XLIII@out}\newcommand\stats@XLIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLIV@out{\{"mean": 1.214229900214069, "std": 2.443644732339022\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLIV@out{1.214229900214069}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLIV@out{2.443644732339022}\else\def\stats@XLIV@out{??}\fi\fi\fi\stats@XLIV@out}\newcommand\stats@XLV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLV@out{\{"mean": 0.6652851932595292, "std": 0.9444693288506714\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLV@out{0.6652851932595292}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLV@out{0.9444693288506714}\else\def\stats@XLV@out{??}\fi\fi\fi\stats@XLV@out}\newcommand\stats@XLVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLVI@out{\{"mean": 2.2961581361167376, "std": 1.9902588271563522\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLVI@out{2.2961581361167376}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLVI@out{1.9902588271563522}\else\def\stats@XLVI@out{??}\fi\fi\fi\stats@XLVI@out}\newcommand\stats@XLVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLVII@out{\{"mean": 1.938145082278047, "std": 1.5620197624637286\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLVII@out{1.938145082278047}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLVII@out{1.5620197624637286}\else\def\stats@XLVII@out{??}\fi\fi\fi\stats@XLVII@out}\newcommand\stats@XLVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLVIII@out{\{"mean": 94.14208165393968, "std": 8.120872618703146\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLVIII@out{94.14208165393968}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLVIII@out{8.120872618703146}\else\def\stats@XLVIII@out{??}\fi\fi\fi\stats@XLVIII@out}\newcommand\stats@XLIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@XLIX@out{\{"mean": 92.98239253273496, "std": 9.462904856958765\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@XLIX@out{92.98239253273496}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@XLIX@out{9.462904856958765}\else\def\stats@XLIX@out{??}\fi\fi\fi\stats@XLIX@out}\newcommand\stats@L[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@L@out{\{"mean": 1.8307136568351885, "std": 2.652931530658601\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@L@out{1.8307136568351885}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@L@out{2.652931530658601}\else\def\stats@L@out{??}\fi\fi\fi\stats@L@out}\newcommand\stats@LI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LI@out{\{"mean": 5.229468421866609, "std": 5.5433969553392135\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LI@out{5.229468421866609}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LI@out{5.5433969553392135}\else\def\stats@LI@out{??}\fi\fi\fi\stats@LI@out}\newcommand\stats@LII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LII@out{\{"mean": 2.8275318786245656, "std": 2.6866561167896887\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LII@out{2.8275318786245656}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LII@out{2.6866561167896887}\else\def\stats@LII@out{??}\fi\fi\fi\stats@LII@out}\newcommand\stats@LIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LIII@out{\{"mean": 2.0505510997680045, "std": 1.8167823562978915\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LIII@out{2.0505510997680045}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LIII@out{1.8167823562978915}\else\def\stats@LIII@out{??}\fi\fi\fi\stats@LIII@out}\newcommand\stats@LIV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LIV@out{\{"mean": 95.2155606928716, "std": 6.823432642887064\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LIV@out{95.2155606928716}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LIV@out{6.823432642887064}\else\def\stats@LIV@out{??}\fi\fi\fi\stats@LIV@out}\newcommand\stats@LV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LV@out{\{"mean": 93.49265301745906, "std": 7.934497826624769\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LV@out{93.49265301745906}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LV@out{7.934497826624769}\else\def\stats@LV@out{??}\fi\fi\fi\stats@LV@out}\newcommand\stats@LVI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LVI@out{\{"mean": 1.2868743196879324, "std": 1.9110147811740117\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LVI@out{1.2868743196879324}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LVI@out{1.9110147811740117}\else\def\stats@LVI@out{??}\fi\fi\fi\stats@LVI@out}\newcommand\stats@LVII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LVII@out{\{"mean": 1.9024102977600428, "std": 2.786503040500623\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LVII@out{1.9024102977600428}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LVII@out{2.786503040500623}\else\def\stats@LVII@out{??}\fi\fi\fi\stats@LVII@out}\newcommand\stats@LVIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LVIII@out{\{"mean": 0.867865724112823, "std": 0.9000931203616069\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LVIII@out{0.867865724112823}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LVIII@out{0.9000931203616069}\else\def\stats@LVIII@out{??}\fi\fi\fi\stats@LVIII@out}\newcommand\stats@LIX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LIX@out{\{"mean": 0.8417458923621104, "std": 0.7908644022261112\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LIX@out{0.8417458923621104}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LIX@out{0.7908644022261112}\else\def\stats@LIX@out{??}\fi\fi\fi\stats@LIX@out}\newcommand\stats@LX[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LX@out{\{"mean": 94.82981224587567, "std": 7.186417040483126\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LX@out{94.82981224587567}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LX@out{7.186417040483126}\else\def\stats@LX@out{??}\fi\fi\fi\stats@LX@out}\newcommand\stats@LXI[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LXI@out{\{"mean": 96.653111411263, "std": 5.410798812779476\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LXI@out{96.653111411263}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LXI@out{5.410798812779476}\else\def\stats@LXI@out{??}\fi\fi\fi\stats@LXI@out}\newcommand\stats@LXII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LXII@out{\{"mean": 9.477527730103349, "std": 3.7853584897791857\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LXII@out{9.477527730103349}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LXII@out{3.7853584897791857}\else\def\stats@LXII@out{??}\fi\fi\fi\stats@LXII@out}\newcommand\stats@LXIII[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\stats@LXIII@out{\{"mean": 10.42505917928366, "std": 3.9728307838983334\}}\else\ifnum\pdfstrcmp{#1}{mean}=0\def\stats@LXIII@out{10.42505917928366}\else\ifnum\pdfstrcmp{#1}{std}=0\def\stats@LXIII@out{3.9728307838983334}\else\def\stats@LXIII@out{??}\fi\fi\fi\stats@LXIII@out}\makeatother

==> data/summary.tex <==
\makeatletter\newcommand\summary[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summary@out{\{"huggingface": \{"num\_artifacts": 2662807, "num\_artifacts\_h": "2.66M", "num\_versions": 2662808, "num\_versions\_h": "2.66M", "num\_packages": 128338, "num\_packages\_h": "128K", "good": 374, "good\_h": "374", "no\_sig": 2660957, "no\_sig\_h": "2.66M", "bad\_sig": 1476, "bad\_sig\_h": "1.48K", "good\_p": "20.2\%", "no\_sig\_p": "99.9\%", "signed\_p": "0.1\%", "signed\_h": "1.85K", "signed": 1850, "bad\_sig\_p": "79.8\%", "no\_pub": 0, "no\_pub\_p": "0.0\%", "no\_pub\_h": "0", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "exp\_pub": 0, "exp\_pub\_p": "0.0\%", "exp\_pub\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0", "rev\_pub": 0, "rev\_pub\_p": "0.0\%", "rev\_pub\_h": "0", "bad\_pub": 0, "bad\_pub\_p": "0.0\%", "bad\_pub\_h": "0"\}, "docker": \{"num\_artifacts": 9517263, "num\_artifacts\_h": "9.52M", "num\_versions": 9517264, "num\_versions\_h": "9.52M", "num\_packages": 91719, "num\_packages\_h": "91.7K", "good": 234805, "good\_h": "235K", "no\_sig": 9282458, "no\_sig\_h": "9.28M", "good\_p": "100.0\%", "no\_sig\_p": "97.5\%", "signed\_p": "2.5\%", "signed\_h": "235K", "signed": 234805, "no\_pub": 0, "no\_pub\_p": "0.0\%", "no\_pub\_h": "0", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "exp\_pub": 0, "exp\_pub\_p": "0.0\%", "exp\_pub\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0", "rev\_pub": 0, "rev\_pub\_p": "0.0\%", "rev\_pub\_h": "0", "bad\_pub": 0, "bad\_pub\_p": "0.0\%", "bad\_pub\_h": "0"\}, "maven": \{"num\_artifacts": 7964488, "num\_artifacts\_h": "7.96M", "num\_versions": 2040617, "num\_versions\_h": "2.04M", "num\_packages": 49959, "num\_packages\_h": "50K", "good": 5138956, "good\_h": "5.14M", "no\_sig": 467071, "no\_sig\_h": "467K", "bad\_sig": 56199, "bad\_sig\_h": "56.2K", "exp\_pub": 1722124, "exp\_pub\_h": "1.72M", "no\_pub": 286610, "no\_pub\_h": "287K", "rev\_pub": 172302, "rev\_pub\_h": "172K", "bad\_pub": 120996, "bad\_pub\_h": "121K", "good\_p": "68.5\%", "no\_sig\_p": "5.9\%", "signed\_p": "94.1\%", "signed\_h": "7.5M", "signed": 7497417, "bad\_sig\_p": "0.7\%", "exp\_pub\_p": "23.0\%", "no\_pub\_p": "3.8\%", "rev\_pub\_p": "2.3\%", "bad\_pub\_p": "1.6\%", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0"\}, "pypi": \{"num\_artifacts": 9677461, "num\_artifacts\_h": "9.68M", "num\_versions": 4829239, "num\_versions\_h": "4.83M", "num\_packages": 205513, "num\_packages\_h": "206K", "good": 60537, "good\_h": "60.5K", "no\_sig": 9556949, "no\_sig\_h": "9.56M", "bad\_sig": 255, "bad\_sig\_h": "255", "exp\_pub": 19241, "exp\_pub\_h": "19.2K", "no\_pub": 19269, "no\_pub\_h": "19.3K", "rev\_pub": 18956, "rev\_pub\_h": "19K", "bad\_pub": 2254, "bad\_pub\_h": "2.25K", "good\_p": "50.2\%", "no\_sig\_p": "98.8\%", "signed\_p": "1.2\%", "signed\_h": "121K", "signed": 120512, "bad\_sig\_p": "0.2\%", "exp\_pub\_p": "16.0\%", "no\_pub\_p": "16.0\%", "rev\_pub\_p": "15.7\%", "bad\_pub\_p": "1.9\%", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0"\}\}}\else\ifnum\pdfstrcmp{#1}{huggingface}=0\let\summary@out\summary@I\else\ifnum\pdfstrcmp{#1}{docker}=0\let\summary@out\summary@II\else\ifnum\pdfstrcmp{#1}{maven}=0\let\summary@out\summary@III\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\summary@out\summary@IV\else\def\summary@out{??}\fi\fi\fi\fi\fi\summary@out}\newcommand\summary@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summary@I@out{\{"num\_artifacts": 2662807, "num\_artifacts\_h": "2.66M", "num\_versions": 2662808, "num\_versions\_h": "2.66M", "num\_packages": 128338, "num\_packages\_h": "128K", "good": 374, "good\_h": "374", "no\_sig": 2660957, "no\_sig\_h": "2.66M", "bad\_sig": 1476, "bad\_sig\_h": "1.48K", "good\_p": "20.2\%", "no\_sig\_p": "99.9\%", "signed\_p": "0.1\%", "signed\_h": "1.85K", "signed": 1850, "bad\_sig\_p": "79.8\%", "no\_pub": 0, "no\_pub\_p": "0.0\%", "no\_pub\_h": "0", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "exp\_pub": 0, "exp\_pub\_p": "0.0\%", "exp\_pub\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0", "rev\_pub": 0, "rev\_pub\_p": "0.0\%", "rev\_pub\_h": "0", "bad\_pub": 0, "bad\_pub\_p": "0.0\%", "bad\_pub\_h": "0"\}}\else\ifnum\pdfstrcmp{#1}{num_artifacts}=0\def\summary@I@out{2662807}\else\ifnum\pdfstrcmp{#1}{num_artifacts_h}=0\def\summary@I@out{2.66M}\else\ifnum\pdfstrcmp{#1}{num_versions}=0\def\summary@I@out{2662808}\else\ifnum\pdfstrcmp{#1}{num_versions_h}=0\def\summary@I@out{2.66M}\else\ifnum\pdfstrcmp{#1}{num_packages}=0\def\summary@I@out{128338}\else\ifnum\pdfstrcmp{#1}{num_packages_h}=0\def\summary@I@out{128K}\else\ifnum\pdfstrcmp{#1}{good}=0\def\summary@I@out{374}\else\ifnum\pdfstrcmp{#1}{good_h}=0\def\summary@I@out{374}\else\ifnum\pdfstrcmp{#1}{no_sig}=0\def\summary@I@out{2660957}\else\ifnum\pdfstrcmp{#1}{no_sig_h}=0\def\summary@I@out{2.66M}\else\ifnum\pdfstrcmp{#1}{bad_sig}=0\def\summary@I@out{1476}\else\ifnum\pdfstrcmp{#1}{bad_sig_h}=0\def\summary@I@out{1.48K}\else\ifnum\pdfstrcmp{#1}{good_p}=0\def\summary@I@out{20.2\%}\else\ifnum\pdfstrcmp{#1}{no_sig_p}=0\def\summary@I@out{99.9\%}\else\ifnum\pdfstrcmp{#1}{signed_p}=0\def\summary@I@out{0.1\%}\else\ifnum\pdfstrcmp{#1}{signed_h}=0\def\summary@I@out{1.85K}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\summary@I@out{1850}\else\ifnum\pdfstrcmp{#1}{bad_sig_p}=0\def\summary@I@out{79.8\%}\else\ifnum\pdfstrcmp{#1}{no_pub}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{no_pub_p}=0\def\summary@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{no_pub_h}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig_p}=0\def\summary@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_sig_h}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{exp_pub}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{exp_pub_p}=0\def\summary@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_pub_h}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_p}=0\def\summary@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_h}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{rev_pub}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{rev_pub_p}=0\def\summary@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{rev_pub_h}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{bad_pub}=0\def\summary@I@out{0}\else\ifnum\pdfstrcmp{#1}{bad_pub_p}=0\def\summary@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{bad_pub_h}=0\def\summary@I@out{0}\else\def\summary@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\summary@I@out}\newcommand\summary@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summary@II@out{\{"num\_artifacts": 9517263, "num\_artifacts\_h": "9.52M", "num\_versions": 9517264, "num\_versions\_h": "9.52M", "num\_packages": 91719, "num\_packages\_h": "91.7K", "good": 234805, "good\_h": "235K", "no\_sig": 9282458, "no\_sig\_h": "9.28M", "good\_p": "100.0\%", "no\_sig\_p": "97.5\%", "signed\_p": "2.5\%", "signed\_h": "235K", "signed": 234805, "no\_pub": 0, "no\_pub\_p": "0.0\%", "no\_pub\_h": "0", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "exp\_pub": 0, "exp\_pub\_p": "0.0\%", "exp\_pub\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0", "rev\_pub": 0, "rev\_pub\_p": "0.0\%", "rev\_pub\_h": "0", "bad\_pub": 0, "bad\_pub\_p": "0.0\%", "bad\_pub\_h": "0"\}}\else\ifnum\pdfstrcmp{#1}{num_artifacts}=0\def\summary@II@out{9517263}\else\ifnum\pdfstrcmp{#1}{num_artifacts_h}=0\def\summary@II@out{9.52M}\else\ifnum\pdfstrcmp{#1}{num_versions}=0\def\summary@II@out{9517264}\else\ifnum\pdfstrcmp{#1}{num_versions_h}=0\def\summary@II@out{9.52M}\else\ifnum\pdfstrcmp{#1}{num_packages}=0\def\summary@II@out{91719}\else\ifnum\pdfstrcmp{#1}{num_packages_h}=0\def\summary@II@out{91.7K}\else\ifnum\pdfstrcmp{#1}{good}=0\def\summary@II@out{234805}\else\ifnum\pdfstrcmp{#1}{good_h}=0\def\summary@II@out{235K}\else\ifnum\pdfstrcmp{#1}{no_sig}=0\def\summary@II@out{9282458}\else\ifnum\pdfstrcmp{#1}{no_sig_h}=0\def\summary@II@out{9.28M}\else\ifnum\pdfstrcmp{#1}{good_p}=0\def\summary@II@out{100.0\%}\else\ifnum\pdfstrcmp{#1}{no_sig_p}=0\def\summary@II@out{97.5\%}\else\ifnum\pdfstrcmp{#1}{signed_p}=0\def\summary@II@out{2.5\%}\else\ifnum\pdfstrcmp{#1}{signed_h}=0\def\summary@II@out{235K}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\summary@II@out{234805}\else\ifnum\pdfstrcmp{#1}{no_pub}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{no_pub_p}=0\def\summary@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{no_pub_h}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig_p}=0\def\summary@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_sig_h}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{exp_pub}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{exp_pub_p}=0\def\summary@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_pub_h}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_p}=0\def\summary@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_h}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{rev_pub}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{rev_pub_p}=0\def\summary@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{rev_pub_h}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{bad_pub}=0\def\summary@II@out{0}\else\ifnum\pdfstrcmp{#1}{bad_pub_p}=0\def\summary@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{bad_pub_h}=0\def\summary@II@out{0}\else\def\summary@II@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\summary@II@out}\newcommand\summary@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summary@III@out{\{"num\_artifacts": 7964488, "num\_artifacts\_h": "7.96M", "num\_versions": 2040617, "num\_versions\_h": "2.04M", "num\_packages": 49959, "num\_packages\_h": "50K", "good": 5138956, "good\_h": "5.14M", "no\_sig": 467071, "no\_sig\_h": "467K", "bad\_sig": 56199, "bad\_sig\_h": "56.2K", "exp\_pub": 1722124, "exp\_pub\_h": "1.72M", "no\_pub": 286610, "no\_pub\_h": "287K", "rev\_pub": 172302, "rev\_pub\_h": "172K", "bad\_pub": 120996, "bad\_pub\_h": "121K", "good\_p": "68.5\%", "no\_sig\_p": "5.9\%", "signed\_p": "94.1\%", "signed\_h": "7.5M", "signed": 7497417, "bad\_sig\_p": "0.7\%", "exp\_pub\_p": "23.0\%", "no\_pub\_p": "3.8\%", "rev\_pub\_p": "2.3\%", "bad\_pub\_p": "1.6\%", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0"\}}\else\ifnum\pdfstrcmp{#1}{num_artifacts}=0\def\summary@III@out{7964488}\else\ifnum\pdfstrcmp{#1}{num_artifacts_h}=0\def\summary@III@out{7.96M}\else\ifnum\pdfstrcmp{#1}{num_versions}=0\def\summary@III@out{2040617}\else\ifnum\pdfstrcmp{#1}{num_versions_h}=0\def\summary@III@out{2.04M}\else\ifnum\pdfstrcmp{#1}{num_packages}=0\def\summary@III@out{49959}\else\ifnum\pdfstrcmp{#1}{num_packages_h}=0\def\summary@III@out{50K}\else\ifnum\pdfstrcmp{#1}{good}=0\def\summary@III@out{5138956}\else\ifnum\pdfstrcmp{#1}{good_h}=0\def\summary@III@out{5.14M}\else\ifnum\pdfstrcmp{#1}{no_sig}=0\def\summary@III@out{467071}\else\ifnum\pdfstrcmp{#1}{no_sig_h}=0\def\summary@III@out{467K}\else\ifnum\pdfstrcmp{#1}{bad_sig}=0\def\summary@III@out{56199}\else\ifnum\pdfstrcmp{#1}{bad_sig_h}=0\def\summary@III@out{56.2K}\else\ifnum\pdfstrcmp{#1}{exp_pub}=0\def\summary@III@out{1722124}\else\ifnum\pdfstrcmp{#1}{exp_pub_h}=0\def\summary@III@out{1.72M}\else\ifnum\pdfstrcmp{#1}{no_pub}=0\def\summary@III@out{286610}\else\ifnum\pdfstrcmp{#1}{no_pub_h}=0\def\summary@III@out{287K}\else\ifnum\pdfstrcmp{#1}{rev_pub}=0\def\summary@III@out{172302}\else\ifnum\pdfstrcmp{#1}{rev_pub_h}=0\def\summary@III@out{172K}\else\ifnum\pdfstrcmp{#1}{bad_pub}=0\def\summary@III@out{120996}\else\ifnum\pdfstrcmp{#1}{bad_pub_h}=0\def\summary@III@out{121K}\else\ifnum\pdfstrcmp{#1}{good_p}=0\def\summary@III@out{68.5\%}\else\ifnum\pdfstrcmp{#1}{no_sig_p}=0\def\summary@III@out{5.9\%}\else\ifnum\pdfstrcmp{#1}{signed_p}=0\def\summary@III@out{94.1\%}\else\ifnum\pdfstrcmp{#1}{signed_h}=0\def\summary@III@out{7.5M}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\summary@III@out{7497417}\else\ifnum\pdfstrcmp{#1}{bad_sig_p}=0\def\summary@III@out{0.7\%}\else\ifnum\pdfstrcmp{#1}{exp_pub_p}=0\def\summary@III@out{23.0\%}\else\ifnum\pdfstrcmp{#1}{no_pub_p}=0\def\summary@III@out{3.8\%}\else\ifnum\pdfstrcmp{#1}{rev_pub_p}=0\def\summary@III@out{2.3\%}\else\ifnum\pdfstrcmp{#1}{bad_pub_p}=0\def\summary@III@out{1.6\%}\else\ifnum\pdfstrcmp{#1}{exp_sig}=0\def\summary@III@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig_p}=0\def\summary@III@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_sig_h}=0\def\summary@III@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig}=0\def\summary@III@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_p}=0\def\summary@III@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_h}=0\def\summary@III@out{0}\else\def\summary@III@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\summary@III@out}\newcommand\summary@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summary@IV@out{\{"num\_artifacts": 9677461, "num\_artifacts\_h": "9.68M", "num\_versions": 4829239, "num\_versions\_h": "4.83M", "num\_packages": 205513, "num\_packages\_h": "206K", "good": 60537, "good\_h": "60.5K", "no\_sig": 9556949, "no\_sig\_h": "9.56M", "bad\_sig": 255, "bad\_sig\_h": "255", "exp\_pub": 19241, "exp\_pub\_h": "19.2K", "no\_pub": 19269, "no\_pub\_h": "19.3K", "rev\_pub": 18956, "rev\_pub\_h": "19K", "bad\_pub": 2254, "bad\_pub\_h": "2.25K", "good\_p": "50.2\%", "no\_sig\_p": "98.8\%", "signed\_p": "1.2\%", "signed\_h": "121K", "signed": 120512, "bad\_sig\_p": "0.2\%", "exp\_pub\_p": "16.0\%", "no\_pub\_p": "16.0\%", "rev\_pub\_p": "15.7\%", "bad\_pub\_p": "1.9\%", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0"\}}\else\ifnum\pdfstrcmp{#1}{num_artifacts}=0\def\summary@IV@out{9677461}\else\ifnum\pdfstrcmp{#1}{num_artifacts_h}=0\def\summary@IV@out{9.68M}\else\ifnum\pdfstrcmp{#1}{num_versions}=0\def\summary@IV@out{4829239}\else\ifnum\pdfstrcmp{#1}{num_versions_h}=0\def\summary@IV@out{4.83M}\else\ifnum\pdfstrcmp{#1}{num_packages}=0\def\summary@IV@out{205513}\else\ifnum\pdfstrcmp{#1}{num_packages_h}=0\def\summary@IV@out{206K}\else\ifnum\pdfstrcmp{#1}{good}=0\def\summary@IV@out{60537}\else\ifnum\pdfstrcmp{#1}{good_h}=0\def\summary@IV@out{60.5K}\else\ifnum\pdfstrcmp{#1}{no_sig}=0\def\summary@IV@out{9556949}\else\ifnum\pdfstrcmp{#1}{no_sig_h}=0\def\summary@IV@out{9.56M}\else\ifnum\pdfstrcmp{#1}{bad_sig}=0\def\summary@IV@out{255}\else\ifnum\pdfstrcmp{#1}{bad_sig_h}=0\def\summary@IV@out{255}\else\ifnum\pdfstrcmp{#1}{exp_pub}=0\def\summary@IV@out{19241}\else\ifnum\pdfstrcmp{#1}{exp_pub_h}=0\def\summary@IV@out{19.2K}\else\ifnum\pdfstrcmp{#1}{no_pub}=0\def\summary@IV@out{19269}\else\ifnum\pdfstrcmp{#1}{no_pub_h}=0\def\summary@IV@out{19.3K}\else\ifnum\pdfstrcmp{#1}{rev_pub}=0\def\summary@IV@out{18956}\else\ifnum\pdfstrcmp{#1}{rev_pub_h}=0\def\summary@IV@out{19K}\else\ifnum\pdfstrcmp{#1}{bad_pub}=0\def\summary@IV@out{2254}\else\ifnum\pdfstrcmp{#1}{bad_pub_h}=0\def\summary@IV@out{2.25K}\else\ifnum\pdfstrcmp{#1}{good_p}=0\def\summary@IV@out{50.2\%}\else\ifnum\pdfstrcmp{#1}{no_sig_p}=0\def\summary@IV@out{98.8\%}\else\ifnum\pdfstrcmp{#1}{signed_p}=0\def\summary@IV@out{1.2\%}\else\ifnum\pdfstrcmp{#1}{signed_h}=0\def\summary@IV@out{121K}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\summary@IV@out{120512}\else\ifnum\pdfstrcmp{#1}{bad_sig_p}=0\def\summary@IV@out{0.2\%}\else\ifnum\pdfstrcmp{#1}{exp_pub_p}=0\def\summary@IV@out{16.0\%}\else\ifnum\pdfstrcmp{#1}{no_pub_p}=0\def\summary@IV@out{16.0\%}\else\ifnum\pdfstrcmp{#1}{rev_pub_p}=0\def\summary@IV@out{15.7\%}\else\ifnum\pdfstrcmp{#1}{bad_pub_p}=0\def\summary@IV@out{1.9\%}\else\ifnum\pdfstrcmp{#1}{exp_sig}=0\def\summary@IV@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig_p}=0\def\summary@IV@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_sig_h}=0\def\summary@IV@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig}=0\def\summary@IV@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_p}=0\def\summary@IV@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_h}=0\def\summary@IV@out{0}\else\def\summary@IV@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\summary@IV@out}\makeatother

==> data/summaryyr.tex <==
\makeatletter\newcommand\summaryyr[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summaryyr@out{\{"huggingface": \{"num\_artifacts": 2020054, "num\_artifacts\_h": "2.02M", "num\_versions": 2020054, "num\_versions\_h": "2.02M", "num\_packages": 100132, "num\_packages\_h": "100K", "good": 296, "good\_h": "296", "no\_sig": 2018818, "no\_sig\_h": "2.02M", "bad\_sig": 940, "bad\_sig\_h": "940", "good\_p": "23.9\%", "no\_sig\_p": "99.9\%", "signed\_p": "0.1\%", "signed\_h": "1.24K", "signed": 1236, "bad\_sig\_p": "76.1\%", "rev\_pub": 0, "rev\_pub\_p": "0.0\%", "rev\_pub\_h": "0", "no\_pub": 0, "no\_pub\_p": "0.0\%", "no\_pub\_h": "0", "bad\_pub": 0, "bad\_pub\_p": "0.0\%", "bad\_pub\_h": "0", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0", "exp\_pub": 0, "exp\_pub\_p": "0.0\%", "exp\_pub\_h": "0"\}, "docker": \{"num\_artifacts": 5003375, "num\_artifacts\_h": "5M", "num\_versions": 5003375, "num\_versions\_h": "5M", "num\_packages": 70024, "num\_packages\_h": "70K", "good": 49083, "good\_h": "49.1K", "no\_sig": 4954292, "no\_sig\_h": "4.95M", "good\_p": "100.0\%", "no\_sig\_p": "99.0\%", "signed\_p": "1.0\%", "signed\_h": "49.1K", "signed": 49083, "rev\_pub": 0, "rev\_pub\_p": "0.0\%", "rev\_pub\_h": "0", "no\_pub": 0, "no\_pub\_p": "0.0\%", "no\_pub\_h": "0", "bad\_pub": 0, "bad\_pub\_p": "0.0\%", "bad\_pub\_h": "0", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0", "exp\_pub": 0, "exp\_pub\_p": "0.0\%", "exp\_pub\_h": "0"\}, "maven": \{"num\_artifacts": 1546815, "num\_artifacts\_h": "1.55M", "num\_versions": 378468, "num\_versions\_h": "378K", "num\_packages": 24110, "num\_packages\_h": "24.1K", "good": 1094256, "good\_h": "1.09M", "no\_sig": 44795, "no\_sig\_h": "44.8K", "bad\_sig": 3730, "bad\_sig\_h": "3.73K", "exp\_pub": 225111, "exp\_pub\_h": "225K", "no\_pub": 109386, "no\_pub\_h": "109K", "rev\_pub": 6765, "rev\_pub\_h": "6.76K", "bad\_pub": 62731, "bad\_pub\_h": "62.7K", "good\_p": "72.9\%", "no\_sig\_p": "2.9\%", "signed\_p": "97.1\%", "signed\_h": "1.5M", "signed": 1502020, "bad\_sig\_p": "0.2\%", "exp\_pub\_p": "15.0\%", "no\_pub\_p": "7.3\%", "rev\_pub\_p": "0.5\%", "bad\_pub\_p": "4.2\%", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0"\}, "pypi": \{"num\_artifacts": 2745869, "num\_artifacts\_h": "2.75M", "num\_versions": 1198749, "num\_versions\_h": "1.2M", "num\_packages": 93233, "num\_packages\_h": "93.2K", "good": 2798, "good\_h": "2.8K", "no\_sig": 2740084, "no\_sig\_h": "2.74M", "bad\_sig": 1, "bad\_sig\_h": "1", "exp\_pub": 384, "exp\_pub\_h": "384", "no\_pub": 1354, "no\_pub\_h": "1.35K", "rev\_pub": 1069, "rev\_pub\_h": "1.07K", "bad\_pub": 179, "bad\_pub\_h": "179", "good\_p": "48.4\%", "no\_sig\_p": "99.8\%", "signed\_p": "0.2\%", "signed\_h": "5.78K", "signed": 5785, "bad\_sig\_p": "0.0\%", "exp\_pub\_p": "6.6\%", "no\_pub\_p": "23.4\%", "rev\_pub\_p": "18.5\%", "bad\_pub\_p": "3.1\%", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0"\}\}}\else\ifnum\pdfstrcmp{#1}{huggingface}=0\let\summaryyr@out\summaryyr@I\else\ifnum\pdfstrcmp{#1}{docker}=0\let\summaryyr@out\summaryyr@II\else\ifnum\pdfstrcmp{#1}{maven}=0\let\summaryyr@out\summaryyr@III\else\ifnum\pdfstrcmp{#1}{pypi}=0\let\summaryyr@out\summaryyr@IV\else\def\summaryyr@out{??}\fi\fi\fi\fi\fi\summaryyr@out}\newcommand\summaryyr@I[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summaryyr@I@out{\{"num\_artifacts": 2020054, "num\_artifacts\_h": "2.02M", "num\_versions": 2020054, "num\_versions\_h": "2.02M", "num\_packages": 100132, "num\_packages\_h": "100K", "good": 296, "good\_h": "296", "no\_sig": 2018818, "no\_sig\_h": "2.02M", "bad\_sig": 940, "bad\_sig\_h": "940", "good\_p": "23.9\%", "no\_sig\_p": "99.9\%", "signed\_p": "0.1\%", "signed\_h": "1.24K", "signed": 1236, "bad\_sig\_p": "76.1\%", "rev\_pub": 0, "rev\_pub\_p": "0.0\%", "rev\_pub\_h": "0", "no\_pub": 0, "no\_pub\_p": "0.0\%", "no\_pub\_h": "0", "bad\_pub": 0, "bad\_pub\_p": "0.0\%", "bad\_pub\_h": "0", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0", "exp\_pub": 0, "exp\_pub\_p": "0.0\%", "exp\_pub\_h": "0"\}}\else\ifnum\pdfstrcmp{#1}{num_artifacts}=0\def\summaryyr@I@out{2020054}\else\ifnum\pdfstrcmp{#1}{num_artifacts_h}=0\def\summaryyr@I@out{2.02M}\else\ifnum\pdfstrcmp{#1}{num_versions}=0\def\summaryyr@I@out{2020054}\else\ifnum\pdfstrcmp{#1}{num_versions_h}=0\def\summaryyr@I@out{2.02M}\else\ifnum\pdfstrcmp{#1}{num_packages}=0\def\summaryyr@I@out{100132}\else\ifnum\pdfstrcmp{#1}{num_packages_h}=0\def\summaryyr@I@out{100K}\else\ifnum\pdfstrcmp{#1}{good}=0\def\summaryyr@I@out{296}\else\ifnum\pdfstrcmp{#1}{good_h}=0\def\summaryyr@I@out{296}\else\ifnum\pdfstrcmp{#1}{no_sig}=0\def\summaryyr@I@out{2018818}\else\ifnum\pdfstrcmp{#1}{no_sig_h}=0\def\summaryyr@I@out{2.02M}\else\ifnum\pdfstrcmp{#1}{bad_sig}=0\def\summaryyr@I@out{940}\else\ifnum\pdfstrcmp{#1}{bad_sig_h}=0\def\summaryyr@I@out{940}\else\ifnum\pdfstrcmp{#1}{good_p}=0\def\summaryyr@I@out{23.9\%}\else\ifnum\pdfstrcmp{#1}{no_sig_p}=0\def\summaryyr@I@out{99.9\%}\else\ifnum\pdfstrcmp{#1}{signed_p}=0\def\summaryyr@I@out{0.1\%}\else\ifnum\pdfstrcmp{#1}{signed_h}=0\def\summaryyr@I@out{1.24K}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\summaryyr@I@out{1236}\else\ifnum\pdfstrcmp{#1}{bad_sig_p}=0\def\summaryyr@I@out{76.1\%}\else\ifnum\pdfstrcmp{#1}{rev_pub}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{rev_pub_p}=0\def\summaryyr@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{rev_pub_h}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{no_pub}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{no_pub_p}=0\def\summaryyr@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{no_pub_h}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{bad_pub}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{bad_pub_p}=0\def\summaryyr@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{bad_pub_h}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig_p}=0\def\summaryyr@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_sig_h}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_p}=0\def\summaryyr@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_h}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{exp_pub}=0\def\summaryyr@I@out{0}\else\ifnum\pdfstrcmp{#1}{exp_pub_p}=0\def\summaryyr@I@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_pub_h}=0\def\summaryyr@I@out{0}\else\def\summaryyr@I@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\summaryyr@I@out}\newcommand\summaryyr@II[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summaryyr@II@out{\{"num\_artifacts": 5003375, "num\_artifacts\_h": "5M", "num\_versions": 5003375, "num\_versions\_h": "5M", "num\_packages": 70024, "num\_packages\_h": "70K", "good": 49083, "good\_h": "49.1K", "no\_sig": 4954292, "no\_sig\_h": "4.95M", "good\_p": "100.0\%", "no\_sig\_p": "99.0\%", "signed\_p": "1.0\%", "signed\_h": "49.1K", "signed": 49083, "rev\_pub": 0, "rev\_pub\_p": "0.0\%", "rev\_pub\_h": "0", "no\_pub": 0, "no\_pub\_p": "0.0\%", "no\_pub\_h": "0", "bad\_pub": 0, "bad\_pub\_p": "0.0\%", "bad\_pub\_h": "0", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0", "exp\_pub": 0, "exp\_pub\_p": "0.0\%", "exp\_pub\_h": "0"\}}\else\ifnum\pdfstrcmp{#1}{num_artifacts}=0\def\summaryyr@II@out{5003375}\else\ifnum\pdfstrcmp{#1}{num_artifacts_h}=0\def\summaryyr@II@out{5M}\else\ifnum\pdfstrcmp{#1}{num_versions}=0\def\summaryyr@II@out{5003375}\else\ifnum\pdfstrcmp{#1}{num_versions_h}=0\def\summaryyr@II@out{5M}\else\ifnum\pdfstrcmp{#1}{num_packages}=0\def\summaryyr@II@out{70024}\else\ifnum\pdfstrcmp{#1}{num_packages_h}=0\def\summaryyr@II@out{70K}\else\ifnum\pdfstrcmp{#1}{good}=0\def\summaryyr@II@out{49083}\else\ifnum\pdfstrcmp{#1}{good_h}=0\def\summaryyr@II@out{49.1K}\else\ifnum\pdfstrcmp{#1}{no_sig}=0\def\summaryyr@II@out{4954292}\else\ifnum\pdfstrcmp{#1}{no_sig_h}=0\def\summaryyr@II@out{4.95M}\else\ifnum\pdfstrcmp{#1}{good_p}=0\def\summaryyr@II@out{100.0\%}\else\ifnum\pdfstrcmp{#1}{no_sig_p}=0\def\summaryyr@II@out{99.0\%}\else\ifnum\pdfstrcmp{#1}{signed_p}=0\def\summaryyr@II@out{1.0\%}\else\ifnum\pdfstrcmp{#1}{signed_h}=0\def\summaryyr@II@out{49.1K}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\summaryyr@II@out{49083}\else\ifnum\pdfstrcmp{#1}{rev_pub}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{rev_pub_p}=0\def\summaryyr@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{rev_pub_h}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{no_pub}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{no_pub_p}=0\def\summaryyr@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{no_pub_h}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{bad_pub}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{bad_pub_p}=0\def\summaryyr@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{bad_pub_h}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig_p}=0\def\summaryyr@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_sig_h}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_p}=0\def\summaryyr@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_h}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{exp_pub}=0\def\summaryyr@II@out{0}\else\ifnum\pdfstrcmp{#1}{exp_pub_p}=0\def\summaryyr@II@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_pub_h}=0\def\summaryyr@II@out{0}\else\def\summaryyr@II@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\summaryyr@II@out}\newcommand\summaryyr@III[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summaryyr@III@out{\{"num\_artifacts": 1546815, "num\_artifacts\_h": "1.55M", "num\_versions": 378468, "num\_versions\_h": "378K", "num\_packages": 24110, "num\_packages\_h": "24.1K", "good": 1094256, "good\_h": "1.09M", "no\_sig": 44795, "no\_sig\_h": "44.8K", "bad\_sig": 3730, "bad\_sig\_h": "3.73K", "exp\_pub": 225111, "exp\_pub\_h": "225K", "no\_pub": 109386, "no\_pub\_h": "109K", "rev\_pub": 6765, "rev\_pub\_h": "6.76K", "bad\_pub": 62731, "bad\_pub\_h": "62.7K", "good\_p": "72.9\%", "no\_sig\_p": "2.9\%", "signed\_p": "97.1\%", "signed\_h": "1.5M", "signed": 1502020, "bad\_sig\_p": "0.2\%", "exp\_pub\_p": "15.0\%", "no\_pub\_p": "7.3\%", "rev\_pub\_p": "0.5\%", "bad\_pub\_p": "4.2\%", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0"\}}\else\ifnum\pdfstrcmp{#1}{num_artifacts}=0\def\summaryyr@III@out{1546815}\else\ifnum\pdfstrcmp{#1}{num_artifacts_h}=0\def\summaryyr@III@out{1.55M}\else\ifnum\pdfstrcmp{#1}{num_versions}=0\def\summaryyr@III@out{378468}\else\ifnum\pdfstrcmp{#1}{num_versions_h}=0\def\summaryyr@III@out{378K}\else\ifnum\pdfstrcmp{#1}{num_packages}=0\def\summaryyr@III@out{24110}\else\ifnum\pdfstrcmp{#1}{num_packages_h}=0\def\summaryyr@III@out{24.1K}\else\ifnum\pdfstrcmp{#1}{good}=0\def\summaryyr@III@out{1094256}\else\ifnum\pdfstrcmp{#1}{good_h}=0\def\summaryyr@III@out{1.09M}\else\ifnum\pdfstrcmp{#1}{no_sig}=0\def\summaryyr@III@out{44795}\else\ifnum\pdfstrcmp{#1}{no_sig_h}=0\def\summaryyr@III@out{44.8K}\else\ifnum\pdfstrcmp{#1}{bad_sig}=0\def\summaryyr@III@out{3730}\else\ifnum\pdfstrcmp{#1}{bad_sig_h}=0\def\summaryyr@III@out{3.73K}\else\ifnum\pdfstrcmp{#1}{exp_pub}=0\def\summaryyr@III@out{225111}\else\ifnum\pdfstrcmp{#1}{exp_pub_h}=0\def\summaryyr@III@out{225K}\else\ifnum\pdfstrcmp{#1}{no_pub}=0\def\summaryyr@III@out{109386}\else\ifnum\pdfstrcmp{#1}{no_pub_h}=0\def\summaryyr@III@out{109K}\else\ifnum\pdfstrcmp{#1}{rev_pub}=0\def\summaryyr@III@out{6765}\else\ifnum\pdfstrcmp{#1}{rev_pub_h}=0\def\summaryyr@III@out{6.76K}\else\ifnum\pdfstrcmp{#1}{bad_pub}=0\def\summaryyr@III@out{62731}\else\ifnum\pdfstrcmp{#1}{bad_pub_h}=0\def\summaryyr@III@out{62.7K}\else\ifnum\pdfstrcmp{#1}{good_p}=0\def\summaryyr@III@out{72.9\%}\else\ifnum\pdfstrcmp{#1}{no_sig_p}=0\def\summaryyr@III@out{2.9\%}\else\ifnum\pdfstrcmp{#1}{signed_p}=0\def\summaryyr@III@out{97.1\%}\else\ifnum\pdfstrcmp{#1}{signed_h}=0\def\summaryyr@III@out{1.5M}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\summaryyr@III@out{1502020}\else\ifnum\pdfstrcmp{#1}{bad_sig_p}=0\def\summaryyr@III@out{0.2\%}\else\ifnum\pdfstrcmp{#1}{exp_pub_p}=0\def\summaryyr@III@out{15.0\%}\else\ifnum\pdfstrcmp{#1}{no_pub_p}=0\def\summaryyr@III@out{7.3\%}\else\ifnum\pdfstrcmp{#1}{rev_pub_p}=0\def\summaryyr@III@out{0.5\%}\else\ifnum\pdfstrcmp{#1}{bad_pub_p}=0\def\summaryyr@III@out{4.2\%}\else\ifnum\pdfstrcmp{#1}{exp_sig}=0\def\summaryyr@III@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig_p}=0\def\summaryyr@III@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_sig_h}=0\def\summaryyr@III@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig}=0\def\summaryyr@III@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_p}=0\def\summaryyr@III@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_h}=0\def\summaryyr@III@out{0}\else\def\summaryyr@III@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\summaryyr@III@out}\newcommand\summaryyr@IV[1][all]{\ifnum\pdfstrcmp{#1}{all}=0\def\summaryyr@IV@out{\{"num\_artifacts": 2745869, "num\_artifacts\_h": "2.75M", "num\_versions": 1198749, "num\_versions\_h": "1.2M", "num\_packages": 93233, "num\_packages\_h": "93.2K", "good": 2798, "good\_h": "2.8K", "no\_sig": 2740084, "no\_sig\_h": "2.74M", "bad\_sig": 1, "bad\_sig\_h": "1", "exp\_pub": 384, "exp\_pub\_h": "384", "no\_pub": 1354, "no\_pub\_h": "1.35K", "rev\_pub": 1069, "rev\_pub\_h": "1.07K", "bad\_pub": 179, "bad\_pub\_h": "179", "good\_p": "48.4\%", "no\_sig\_p": "99.8\%", "signed\_p": "0.2\%", "signed\_h": "5.78K", "signed": 5785, "bad\_sig\_p": "0.0\%", "exp\_pub\_p": "6.6\%", "no\_pub\_p": "23.4\%", "rev\_pub\_p": "18.5\%", "bad\_pub\_p": "3.1\%", "exp\_sig": 0, "exp\_sig\_p": "0.0\%", "exp\_sig\_h": "0", "goodbad\_sig": 0, "goodbad\_sig\_p": "0.0\%", "goodbad\_sig\_h": "0"\}}\else\ifnum\pdfstrcmp{#1}{num_artifacts}=0\def\summaryyr@IV@out{2745869}\else\ifnum\pdfstrcmp{#1}{num_artifacts_h}=0\def\summaryyr@IV@out{2.75M}\else\ifnum\pdfstrcmp{#1}{num_versions}=0\def\summaryyr@IV@out{1198749}\else\ifnum\pdfstrcmp{#1}{num_versions_h}=0\def\summaryyr@IV@out{1.2M}\else\ifnum\pdfstrcmp{#1}{num_packages}=0\def\summaryyr@IV@out{93233}\else\ifnum\pdfstrcmp{#1}{num_packages_h}=0\def\summaryyr@IV@out{93.2K}\else\ifnum\pdfstrcmp{#1}{good}=0\def\summaryyr@IV@out{2798}\else\ifnum\pdfstrcmp{#1}{good_h}=0\def\summaryyr@IV@out{2.8K}\else\ifnum\pdfstrcmp{#1}{no_sig}=0\def\summaryyr@IV@out{2740084}\else\ifnum\pdfstrcmp{#1}{no_sig_h}=0\def\summaryyr@IV@out{2.74M}\else\ifnum\pdfstrcmp{#1}{bad_sig}=0\def\summaryyr@IV@out{1}\else\ifnum\pdfstrcmp{#1}{bad_sig_h}=0\def\summaryyr@IV@out{1}\else\ifnum\pdfstrcmp{#1}{exp_pub}=0\def\summaryyr@IV@out{384}\else\ifnum\pdfstrcmp{#1}{exp_pub_h}=0\def\summaryyr@IV@out{384}\else\ifnum\pdfstrcmp{#1}{no_pub}=0\def\summaryyr@IV@out{1354}\else\ifnum\pdfstrcmp{#1}{no_pub_h}=0\def\summaryyr@IV@out{1.35K}\else\ifnum\pdfstrcmp{#1}{rev_pub}=0\def\summaryyr@IV@out{1069}\else\ifnum\pdfstrcmp{#1}{rev_pub_h}=0\def\summaryyr@IV@out{1.07K}\else\ifnum\pdfstrcmp{#1}{bad_pub}=0\def\summaryyr@IV@out{179}\else\ifnum\pdfstrcmp{#1}{bad_pub_h}=0\def\summaryyr@IV@out{179}\else\ifnum\pdfstrcmp{#1}{good_p}=0\def\summaryyr@IV@out{48.4\%}\else\ifnum\pdfstrcmp{#1}{no_sig_p}=0\def\summaryyr@IV@out{99.8\%}\else\ifnum\pdfstrcmp{#1}{signed_p}=0\def\summaryyr@IV@out{0.2\%}\else\ifnum\pdfstrcmp{#1}{signed_h}=0\def\summaryyr@IV@out{5.78K}\else\ifnum\pdfstrcmp{#1}{signed}=0\def\summaryyr@IV@out{5785}\else\ifnum\pdfstrcmp{#1}{bad_sig_p}=0\def\summaryyr@IV@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_pub_p}=0\def\summaryyr@IV@out{6.6\%}\else\ifnum\pdfstrcmp{#1}{no_pub_p}=0\def\summaryyr@IV@out{23.4\%}\else\ifnum\pdfstrcmp{#1}{rev_pub_p}=0\def\summaryyr@IV@out{18.5\%}\else\ifnum\pdfstrcmp{#1}{bad_pub_p}=0\def\summaryyr@IV@out{3.1\%}\else\ifnum\pdfstrcmp{#1}{exp_sig}=0\def\summaryyr@IV@out{0}\else\ifnum\pdfstrcmp{#1}{exp_sig_p}=0\def\summaryyr@IV@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{exp_sig_h}=0\def\summaryyr@IV@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig}=0\def\summaryyr@IV@out{0}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_p}=0\def\summaryyr@IV@out{0.0\%}\else\ifnum\pdfstrcmp{#1}{goodbad_sig_h}=0\def\summaryyr@IV@out{0}\else\def\summaryyr@IV@out{??}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\summaryyr@IV@out}\makeatother
